Multiplayer Homicidal Chauffeur Reach-Avoid Games: A Pursuit Enclosure Function Approach

This paper presents a multiplayer Homicidal Chauffeur reach-avoid differential game, which involves Dubins-car pursuers and simple-motion evaders. The goal of the pursuers is to cooperatively protect a planar convex region from the evaders, who strive to reach the region. We propose a cooperative strategy for the pursuers based on subgames for multiple pursuers against one evader and optimal task allocation. We introduce pursuit enclosure functions (PEFs) and propose a new enclosure region pursuit (ERP) winning approach that supports forward analysis for the strategy synthesis in the subgames. We show that if a pursuit coalition is able to defend the region against an evader under the ERP winning, then no more than two pursuers in the coalition are necessarily needed. We also propose a steer-to-ERP approach to certify the ERP winning and synthesize the ERP winning strategy. To implement the strategy, we introduce a positional PEF and provide the necessary parameters, states, and strategies that ensure the ERP winning for both one pursuer and two pursuers against one evader. Additionally, we formulate a binary integer program using the subgame outcomes to maximize the captured evaders in the ERP winning for the pursuit task allocation. Finally, we propose a multiplayer receding-horizon strategy where the ERP winnings are checked in each horizon, the task is allocated, and the strategies of the pursuers are determined. Numerical examples are provided to illustrate the results.

==> single_evader.tex <==
\section{Enclosure Region Pursuit Winning and Coalition Reduction against One Evader}\label{sec:ERP-reduction}

It is hard to deal with multiple pursuers against multiple evaders directly due to complicated cooperation among team members and the lack of sensible matching rules between the players of different teams \citep{RY-XD-ZS-YZ-FB:19,MC-ZZ-CJT:17,DS-VK:20,DS-VK:18}. As an alternative, we split the whole game into many subgames, from which cooperative strategies and matching rules are extracted, thus comprising the team strategies. 
% after the mixture. 
The subgames considered in this section focus on multiple pursuers and a single evader.

We first introduce the following definitions and notations specialized for multiple pursuers. For any non-empty index set $c \in 2^{\{1,\dots,N_p\}}$, let $P_c=\{P_i \in \pteam \mid i \in c \}$ be an element of $2^{\pteam}$, and we refer to $P_c$ as a \emph{pursuit coalition} containing pursuer $P_i$ if $i \in c$. 
% In other words, $P_c$ is a pursuit coalition with its members specified by the index set $c$. 
We denote by $X_c$ and $U_c$ the states (positions and headings) and control inputs of all pursuers in $P_c$, respectively, i.e., $X_c = \{(\bm{x}_{P_i}, \theta_{P_i})\}_{i \in c}$ and $U_c = \{ u_{P_i}\}_{i \in c}$. 
% For any $\theta \in \mathbb{R}$, let $\pdirect = [\cos \theta, \sin \theta]^{\top} \in \partial\mathbb{S}^2$. 

\subsection{Enclosure region pursuit winning}

Consider a subgame between a pursuit coalition $P_c$ and an evader $E_j$, in which $P_c$ wins the game if $E_j$ can never reach $\goal$ before being captured, while $E_j$ wins if it reaches $\goal$ prior to the capture. Our goal in this section is to determine, given the initial states, who wins the game. A complete solution to this qualitative problem involves solving an induced HJI equation numerically. However, the standard HJI method can only efficiently handle systems of up to five states \citep{MC-SLH-MSV-SB-CJT:18}, while this subgame has $3|c|+2$ states.
% for multiple pursuers and one evader. 
Note that $P_c$ wins the game in two possible ways: capture $E_j$ in $\play$ or infinitely delay $E_j$'s entry into $\play$. We instead establish a stronger winning condition that a dynamic region containing the evader consistently stays outside the goal region before the capture. This motivates our function-induced pursuit winning and strategies below. Before that, we introduce a class of functions. 

\begin{defi}\label{defi:PEF}{\rm (Pursuit enclosure function).}
For $P_i \in \pteam$ and $E_j \in \eteam$, let $X_{ij} = (\bm{x}_{P_i}, \theta_{P_i}, \bm{x}_{E_j})$ and $\mathcal{S}_{ij} = \{ X_{ij} \in \mathbb{R}^2 \times [0, 2\pi) \times \mathbb{R}^2 \mid \enVert[0]{\bm{x}_{P_i}-\bm{x}_{E_j}}_2 > r_i \}$. Then, a function $f:\mathbb{R}^2 \times \mathcal{S}_{ij}\to\mathbb{R}$ is a \emph{pursuit enclosure function (PEF)} if for each $X_{ij} \in \mathcal{S}_{ij}$, it satisfies the following conditions:
\begin{enumerate}
    \item\label{itm:PEF-defi-1} $\mathbb{E}(X_{ij};f)=\{\bm{x}\in\mathbb{R}^2\,|\,f(\bm{x},X_{ij})\ge0\}$ is compact and strictly convex. We call $\mathbb{E}(X_{ij};f)$ the \emph{enclosure region} of $P_i$ against $E_j$ via $f$;
    
    \item\label{itm:PEF-defi-2} 
    if $ f(\bm{x},X_{ij}) = 0$, then $f$ is differentiable in both $\bm{x}$ and $X_{ij}$;
    
    % \item\label{itm:PEF-defi-2} there exist two functions $\sigma^d, \sigma^u : \mathbb{R}^2 \times \mathbb{R}^2 \to [0, 2 \pi) $ without intersection and splitting $\mathcal{C}$ into three disjoint subspaces 
    % \begin{equation*}
    %     \begin{aligned}
    %         \mathcal{C}_N & = \{ X \in \mathcal{C} \mid \theta_P \neq  \sigma^d(\bm{x}_P, \bm{x}_E), \theta_P \neq  \sigma^u(\bm{x}_P, \bm{x}_E) \}, \\
    %         \mathcal{C}_D & = \{ X \in \mathcal{C} \mid \theta_P =  \sigma^d(\bm{x}_P, \bm{x}_E) \}, \\
    %         \mathcal{C}_U & = \{ X \in \mathcal{C} \mid \theta_P =  \sigma^u(\bm{x}_P, \bm{x}_E) \}.
    %     \end{aligned}
    % \end{equation*}
    % There exists a constant $\epsilon \in \mathbb{R}_{>0}$ such that if $X \in \mathcal{C}_N$ and $ \envert[0]{f(\bm{x},X)} < \epsilon$, then $f$ is differentiable in $\bm{x}$, $\bm{x}_P$, $\theta_P$ and $\bm{x}_E$, and if $X \in \mathcal{C}_U$ and $ \envert[0]{f(\bm{x},X)} < \epsilon$, then
    % \begin{equation*}
    %     f^u(\bm{x}, \bm{x}_P, \bm{x}_E) \coloneqq f(\bm{x}, \bm{x}_P, \sigma^u(\bm{x}_P, \bm{x}_E), \bm{x}_E)
    % \end{equation*}
    % is differentiable in $\bm{x}$, $\bm{x}_P$, and $\bm{x}_E$;
    
    % \item in the small neighborhoods of $\mathcal{C}_D$ and $\mathcal{C}_U$ except themselves, 
    % \begin{equation}
    %     [\sigma^d_P, -1, \sigma^d_E] \cdot F > 0, \quad [\sigma^u_P, -1, \sigma^u_E] \cdot F < 0,
    % \end{equation}
    % where $F = [\dot{\bm{x}}_P, \dot{\theta}, \dot{\bm{x}}_E]^{\top}$ for any $u_P$ and $\bm{u}_E$, $\sigma^d_{\textup{opt}} = \pd{\sigma^d}{\bm{x}_\textup{opt}}$ and $\sigma^u_{\textup{opt}} = \pd{\sigma^u}{\bm{x}_\textup{opt}}$ for $\textup{opt} \in \{ P, E\}$;
    
    \item \label{itm:PEF-defi-3}$f(\bm{x}_{E_j},X_{ij})\ge0$.
\end{enumerate}
% for all $\bm{y}\in\mathbb{R}^2$, $\theta \in \mathbb{R}$ and $\bm{z}\in\mathbb{R}^2$ such that $\enVert[0]{\bm{y}-\bm{z}}_2 > r$.
\end{defi}

% \begin{defi}\label{defi:PEF}{\rm (Pursuit enclosure function).}
% For a pursuer $P \in \pteam$ with capture radius $r$ and, let $\mathcal{C} = \{ (\bm{y}, \theta, \bm{z}) \in \mathbb{R}^2 \times \mathbb{R} \times \mathbb{R}^2 \mid \enVert[0]{\bm{y}-\bm{z}}_2 > r \}$. Then, a function $f:\mathbb{R}^2 \times \mathcal{C}\to\mathbb{R}$ is a \emph{pursuit enclosure function (PEF)} if for each $(\bm{y}, \theta, \bm{z}) \in \mathcal{C}$, it satisfies the following conditions:
% \begin{enumerate}
%     \item\label{itm:PEF-defi-1} $\mathbb{E}(\bm{y},\theta,\bm{z};f)=\{\bm{x}\in\mathbb{R}^2\,|\,f(\bm{x},\bm{y},\theta,\bm{z})\ge0\}$ is compact and strictly convex. We call $\mathbb{E}(\bm{y},\theta,\bm{z};f)$ the enclosure region of $P$ via $f$;
    
%     \item\label{itm:PEF-defi-2} there exist two functions $\sigma_d, \sigma_u : \mathbb{R}^2 \times \mathbb{R}^2 \to \partial \mathbb{S}^2 $ without intersection and splitting $\mathcal{C}$ into three disjoint subspaces 
%     \begin{equation*}
%         \begin{aligned}
%             \mathcal{C}_N & = \{ (\bm{y}, \theta, \bm{z}) \in \mathcal{C} \mid \pdirect \neq  \sigma_d(\bm{y}, \bm{z}), \pdirect \neq  \sigma_u(\bm{y}, \bm{z}) \}, \\
%             \mathcal{C}_D & = \{ (\bm{y}, \theta, \bm{z}) \in \mathcal{C} \mid \pdirect =  \sigma_d(\bm{y}, \bm{z}) \}, \\
%             \mathcal{C}_U & = \{ (\bm{y}, \theta, \bm{z}) \in \mathcal{C} \mid \pdirect =  \sigma_u(\bm{y}, \bm{z}) \}.
%         \end{aligned}
%     \end{equation*}
%     Then, there exists a constant $\epsilon \in \mathbb{R}_{>0}$ such that if $ \envert[0]{f(\bm{x},\bm{y},\theta,\bm{z})} < \epsilon$, then $f$ is differentiable in $\bm{x}$, $\bm{y}$, $\theta$ and $\bm{z}$ over the set $\mathcal{C}_N$, $\mathcal{C}_D$ and $\mathcal{C}_U$ respectively;
    
%     \item if $u_{P}$ is adopted by $P$ in $ \mathcal{C}_N$, then 
%     % and $f^{\sigma} (\bm{x},\bm{y}, \bm{z}) \coloneqq f(\bm{x},\bm{y},\sigma(\bm{y}, \bm{z}),\bm{z})$ is differentiable in $\bm{x}$, $\bm{y}$ and $\bm{z}$ over the set $\mathcal{C}_A$. 
   
    
%     %  \item\label{itm:PEF-defi-2} there exists a constant $\epsilon \in \mathbb{R}_{>0}$ and a function $\sigma : \mathbb{R}^2 \times \mathbb{R}^2 \to \mathbb{R}^2 $ such that $f(\bm{x},\bm{y},\pdirect,\bm{z})$ is differentiable in $\bm{x}$, $\bm{y}$, $\theta$ and $\bm{z}$ over the set $\{(\bm{x},\bm{y},\theta,\bm{z}) \mid \envert[0]{f(\bm{x},\bm{y},\pdirect,\bm{z})} \leq \epsilon, \pdirect \neq \sigma(\bm{y}, \bm{z}) \}$. If $\pdirect = \sigma(\bm{y}, \bm{z})$, then $f^{\sigma} (\bm{x},\bm{y}, \bm{z}) \coloneqq f(\bm{x},\bm{y},\sigma(\bm{y}, \bm{z}),\bm{z})$ is differentiable in $\bm{x}$, $\bm{y}$ and $\bm{z}$ over the set $\{(\bm{x},\bm{y}, \bm{z}) \mid \envert[0]{f^{\sigma}(\bm{x},\bm{y}, \bm{z})} \leq \epsilon\}$. We call $\sigma$ absorbing function of $P$ via $f$.
    
%     % \item\label{itm:PEF-defi-2} $f(\bm{x},\bm{y},\theta,\bm{z})$ is continuously differentiable in $\bm{x}$, $\bm{y}$ and $\bm{z}$, and piecewise continuously differentiable in $\theta$, over the subspace $\{(\bm{x},\bm{y},\theta,\bm{z}) \mid f(\bm{x},\bm{y},\theta,\bm{z}) \ge 0 \}$;
    
%     \item \label{itm:PEF-defi-3}$f(\bm{z},\bm{y},\theta,\bm{z})\ge0$.
% \end{enumerate}
% % for all $\bm{y}\in\mathbb{R}^2$, $\theta \in \mathbb{R}$ and $\bm{z}\in\mathbb{R}^2$ such that $\enVert[0]{\bm{y}-\bm{z}}_2 > r$.
% \end{defi}



%  We are now ready to define new pursuit winning conditions based on the PEFs. Let $X_{cj}=(\bm{x}_s,\bm{x}_{E_j})$ be the state of the system comprising of $P_c$ and $E_j$. We assign each pair $(P_i,E_j)$ a PEF $f_{ij}$ with $\alpha = \alpha_{ij}$ and $r= r_i$. For any $\bm{x} \in \mathbb{R}^2$ and $X_{cj} \in \mathcal{C}_s^c$, we define the function
% \begin{equation*}
%     h(\bm{x},X_{cj})=\min_{i\in s}f_{ij}(\bm{x},\bm{x}_{P_i},\theta_{P_i},\bm{x}_{E_j}).
% \end{equation*}
% The function $h$ is called the \emph{merged PPF} of all $f_{ij}$ $(i \in c)$. We define $\mathbb{E}(X_{cj};h)=\cap_{i \in c}\mathbb{E}(\bm{x}_{P_i},\theta_{P_i},\bm{x}_{E_j};f_i)=\{\bm{x}\in\mathbb{R}^2\,|\,h(\bm{x},X_{cj})\ge0\}$, which is nonempty as $\bm{x}_E\in\mathbb{E}(X_{cj};h)$ for all $X_{cj} \in \mathcal{C}_s^c$. The set $\mathbb{E}(X_{cj};h)$ is also compact and strictly convex. 

% Initialized to an initial state $X_{cj}$ at time $t_0\ge0$, the state of the system at time $t\ge t_0$ under the control pair $(\bm{u}_s,\bm{u}_E)$ is denoted by $X_{cj}^t(\bm{u}_s,\bm{u}_E;t_0)$. We have $X_{cj}^{t_0}(\bm{u}_s,\bm{u}_E;t_0)=X_{cj}$. Unless for clarity, we will omit the arguments in $X_{cj}^t$.

% \begin{defi}[$h$-pursuit winning]\label{defi:merged-h-pursuit-winning}
% Given a merged PPF $h$, a state $X_{cj}$ is \emph{$h$-pursuit winning} if, initialized to $X_{cj}$ at $t_0$, there exists a pursuit strategy $\bm{u}_s(\cdot)$ for the pursuit coalition $P_c$ such that for all $t \ge t_0$, then $\rho(\mathbb{E}(X_{cj}^t;h),\goal)\ge0$ or $X_{cj}^t \in \mathcal{C}_s$, regardless of the evader strategy $\bm{u}_E(\cdot)\in\mathbb{U}^2$. Such a strategy $\bm{u}_s$ is called an $h$-pursuit winning strategy of $X_{cj}$. 
% \end{defi}

% An $h$-pursuit winning strategy $\bm{u}_s$ of $X_{cj}$ is \emph{monotonic} if initialized to $X_{cj}$ at $t_0$, then for all $t \ge t_0$ and all $X_{cj} \in \mathcal{C}_s^c$,  $\od{}{t}\rho(\mathbb{E}(X_{cj};h),\goal)\ge0$ holds, regardless of $E_j$'s strategy.

% \begin{defi}[Interception and projection points]\label{defi:interception-point}
% Given a merged PPF $h$, if $X_{cj} \in \mathcal{C}_s^c$ and $\rho(\mathbb{E}(X_{cj};h),\goal)\ge0$, let the interception point $\bm{x}_{I} \in \mathbb{E}(X_{cj};h)$ and the projection point $\bm{x}_{G} \in \goal$ be the unique pair such that $\enVert[0]{\bm{x}_I-\bm{x}_G}_2=\rho(\mathbb{E}(X_{cj};h),\goal)$, that is, the pair $(\bm{x}_I,\bm{x}_G)$ is the unique solution of the convex problem
% \begin{equation}\label{eq:convex-pbm-IG}
% \begin{aligned}
% \mathcal{P}_{sj} : \; & \underset{(\bm{x},\bm{y})\in\mathbb{R}^2\times\mathbb{R}^2}{\textup{minimize}}
% 	&& \rho(\bm{x},\bm{y})\\
% 	&\textup{ subject to}&& f_{ij}(\bm{x},X_{ij})\ge 0,\; g(\bm{y})\le 0, \; \forall i\in s.
% \end{aligned}
% \end{equation}
% \end{defi}

% \begin{defi}[$f$-no-approaching winning]
% Given a PEF $f$ and a set of states $\mathcal{X} \subset \mathcal{A}$, a pursuer $P$ achieves $f$-no-approaching winning against an evader $E$ over the state space $\mathcal{X}$, if there exists a pursuit strategy $u_{P}(\cdot)$ such that $\od{}{t}{\varrho}(X, f) \ge 0$ for all $X \in \mathcal{X}$, regardless of $\bm{u}_E$. Such a strategy $u_{P}$ is called an $f$-no-approaching winning strategy over $\mathcal{X}$. 
% \end{defi}
%  We call $\sigma_d$ and $\sigma_u$ the dispersal and universal functions respectively, and $\mathcal{C}_N$, $\mathcal{C}_D$ and $\mathcal{C}_U$ the induced non-singular subspace, dispersal and universal surfaces, respectively. The motivation for these definitions will be clear in Section \ref{subsec:strategy-one-pursuer}.
 
The conditions (\ref{itm:PEF-defi-1}) and (\ref{itm:PEF-defi-3}) imply that the evader $E_j$ is contained in the enclosure region $\mathbb{E}(X_{ij};f)$ (green region in Fig. \ref{fig:ERP-winning}). We are now ready to define a new class of pursuit winning conditions based on the PEFs. Let $X_{cj}=(X_c,\bm{x}_{E_j})$ be the state of the system comprising of $P_c$ and $E_j$, and $\mathcal{S}_{cj}= \{ X_{cj} \mid \forall i \in c, \|\bm{x}_{P_i} - \bm{x}_{E_j}\|_2 > r_i \} $ be the set of states such that $E_j$ is not captured by any pursuer in $P_c$. 
%  Specially for one pursuer $P_i$ against $E_j$, $X_{ij} = ( \bm{x}_{P_i}, \theta_{P_i},\bm{x}_{E_j} )$ and $\mathcal{S}_{ij} = \{ X_{ij} \mid \|\bm{x}_{P_i} - \bm{x}_{E_j}\|_2 > r_i \} $. 
 Unless otherwise stated we assume that $X_{cj} \in \mathcal{S}_{cj}$ hereinafter. Suppose that $P_c$ is endowed with a set $f_c$ of PEFs, where $f_c = \{f_i\}_{i \in c}$ and $f_i$ is a PEF for pursuer $P_i$ $(i \in c)$, and we omit the subscript $j$ for PEFs for simplicity. 
 % Since $\| \bm{x}_{P_i} - \bm{x}_{E_j} \|_2 > r_i$ using $X_{cj} \in \mathcal{S}_{cj}$, $f_i(\bm{x},X_{ij})$ is well-defined over $\mathcal{S}_{cj}$ for all $i \in c$.
 Then, the intersection of the enclosure regions of $P_i$ against $E_j$ via $f_i$ for all $i \in c$, is
 \begin{equation*}
\begin{aligned}
   \mathbb{E}(X_{cj}; f_c)  &  \triangleq \cap_{i \in c}\mathbb{E}(X_{ij};f_i) \\
   & = \{\bm{x}\in\mathbb{R}^2 \,|\, f_i(\bm{x},X_{ij}) \ge 0, i \in c\}.
\end{aligned}
 \end{equation*}
By \defiref{defi:PEF}, $\mathbb{E}(X_{cj}; f_c)$ is nonempty because $\bm{x}_{E_j} \in \mathbb{E}(X_{cj}; f_c)$, and it is compact and strictly convex. Letting
\[\varrho(X_{cj}; f_c) \triangleq d( \mathbb{E}(X_{cj}; f_c), \goal )\]
be the distance between the region $\mathbb{E}(X_{cj}; f_c)$ and the goal region, we introduce \emph{safe distance} for $P_c$ against $E_j$.

\begin{defi}\label{defi:safe-distance}{\rm (Safe distance).} Consider a pursuit coalition $P_c$ and an evader $E_j$. Given a set $f_c$ of PEFs, the \emph{safe distance} of a state $X_{cj} \in \mathcal{S}_{cj}$ under $f_c$ is $\varrho (X_{cj}; f_c)$.
\end{defi}
Since $\bm{x}_{E_j} \in \mathbb{E}(X_{cj}; f_c)$, then $d(\bm{x}_{E_j}, \goal) \ge \varrho (X_{cj}; f_c)$ for all $X_{cj} \in \mathcal{S}_{cj}$. This implies that if the safe distance is positive, i.e., $\varrho (X_{cj}; f_c) > 0$, then $E_j$ resides outside of $\goal$. Let $X_{cj}^{t}$ be the system state at $t \ge 0$ when starting from $X_{cj}$ under control inputs $U_c$ and $\bm{u}_{E_j}$.
% , and we omit $U_c$ and $\bm{u}_{E_j}$ unless otherwise specified. 
Next, we introduce a new pursuit winning  based on the safe distance.

% In this paper, we focus on states with non-negative safe distance, i.e., $\mathcal{A}_{sj} = \{ X_{cj} \in \mathcal{S}_{cj}\mid \varrho(X_{cj}; f_c) \ge 0 \}$, by which our new class of pursuit wining conditions is introduced below.
% Since $\bm{x}_{E_j} \in \mathbb{E}(X_{cj}; f_c)$, then $\rho(\bm{x}_{E_j}, \goal) \ge \varrho (X_{cj}; f_c)$ for all $X_{cj} \in \mathcal{S}_{cj}$. This implies that the greater $\varrho (X_{cj}; f_c)$ is, the safer $\goal$ is for $P_c$ against $E_j$. In this paper, we focus on states with non-negative safe distance, i.e., $\mathcal{A}_{sj} = \{ X_{cj} \in \mathcal{S}_{cj}\mid \varrho(X_{cj}; f_c) \ge 0 \}$, by which our new class of pursuit wining conditions is introduced below.
 
% \begin{defi}[$f$-no-approaching winning]
% Given a PEF $f$ and a set of states $\mathcal{X} \subset \mathcal{A}$, a pursuer $P$ achieves $f$-no-approaching winning against an evader $E$ over the state space $\mathcal{X}$, if there exists a pursuit strategy $u_{P}(\cdot)$ such that $\od{}{t}{\varrho}(X, f) \ge 0$ for all $X \in \mathcal{X}$, regardless of $\bm{u}_E$. Such a strategy $u_{P}$ is called an $f$-no-approaching winning strategy over $\mathcal{X}$. 
% \end{defi}

\begin{defi}{\rm(ERP winning state and strategy).}\label{defi:ERP-winning}
Given a set $f_c$ of PEFs, a state $X_{cj} \in \mathcal{S}_{cj}$ is an enclosure region pursuit (ERP) winning state, if there exists a pursuit strategy $U_c$ of $P_c$ such that the safe distance is positive from $X_{cj}$ for all $t \ge 0$, i.e., $\varrho (X_{cj}^t; f_c)  > 0$ for all $t \ge 0$, regardless of $\bm{u}_{E_j}$. Such a strategy $U_c$ is called an ERP winning strategy. 
\end{defi}

% \begin{defi}{\rm (Enclosure region winning).}
% Given a set $f_c$ of PEFs and a set of states $\mathcal{X} \subset \mathcal{A}_{sj}$, $P_c$ achieves no-approaching winning against $E_j$ over $\mathcal{X}$, if there exists a pursuit strategy $U_c$ of $P_c$ such that $\od{}{t} \varrho (X_{cj}; f_c) \ge 0$ for all $X_{cj} \in \mathcal{X}$, regardless of $\bm{u}_{E_j}$. Such a strategy $U_c$ is called no-approaching winning strategy over $\mathcal{X}$. 
% \end{defi}

By \defiref{defi:ERP-winning}, if a state $X_{cj}$ is an ERP winning state, then the pursuit coalition can ensure that from this state, the evader can never enter $\goal$ prior to the capture, by using the ERP winning strategy, as depicted in Fig. \ref{fig:ERP-winning}. Since $\mathbb{E}(X_{cj}; f_c)$ is strictly convex and $\goal$ is convex, computing the safe distance $\varrho (X_{cj}; f_c)$ involves solving a convex optimization problem.

% Since $\mathbb{E}(X_{cj}; f_c)$ is strictly convex and $\goal$ is convex, we can compute $\varrho (X_{cj}; f_c)$ by solving a convex optimization problem, with which we will show that determining the sign of $\od{}{t} \varrho (X_{cj}; f_c)$ as required by the winning condition, is accessible. 

% For simplicity, we denote by $X_{ij}$ the system state for $P_i$ and $E_j$, i.e., $X_{ij} = ( \bm{x}_{P_i},\theta_{P_i},\bm{x}_{E_j} )$, and for a PEF $f$, refer to $f(\bm{x}, \bm{x}_{P_i}, \bm{e}_{\theta_{P_i}},\bm{x}_{E_j} )$ as $f(\bm{x}, X_{ij})$.

\begin{defi}\label{defi:closest-point-mapping}{\rm (Computing the safe distance).}
Given a set $f_c$ of PEFs and a state $X_{cj} \in \mathcal{S}_{cj}$, let $(\bm{x}_I, \bm{x}_G)$ be the solution of the convex optimization problem $\mathcal{P}(X_{cj})$:
\begin{equation}\label{eq:convex-pbm-IG}
\begin{aligned}
    & \underset{(\bm{x},\bm{y})\in\mathbb{R}^2\times\mathbb{R}^2}{\textup{minimize}}
	&& d (\bm{x},\bm{y})\\
	&\textup{ subject to}&& f_i(\bm{x},X_{ij})\ge 0,\; g(\bm{y})\le 0, \; \forall i\in c.
\end{aligned}
\end{equation}
Then, the safe distance is $\varrho (X_{cj}; f_c) = d (\bm{x}_I, \bm{x}_G)$.
% Then, the function $\eta: \mathcal{S}_{cj}\to \mathbb{R}^2$ such that $\eta(X_{cj}) = \bm{x}_I$ for all $X_{cj} \in \mathcal{S}_{cj}$, is the \emph{closest-point mapping} via $f_c$.
\end{defi}
% If $\rho(\bm{x}_I, \bm{x}_G) > 0$, then the safe distance $\varrho (X_{cj}; f_c)$ is positive and equal to $\rho(\bm{x}_I, \bm{x}_G)$. If $\rho(\bm{x}_I, \bm{x}_G) = 0$, we distinguish between zero and negative safe distances from a practical view as follows: Take a small constant $\epsilon \in \mathbb{R}_{>0}$ and sample points with distance to $\bm{x}_I$ less than $\epsilon$. If a sampled point $\bm{x}$ distinct from $\bm{x}_I$ is such that $(\bm{x}, \bm{x})$ is feasible in \eqref{eq:convex-pbm-IG}, then $\varrho (X_{cj}; f_c)$ is negative (i.e., $-\infty$), and zero otherwise.


\begin{figure}
    \centering
\includegraphics[width=0.9\hsize]{figures/PEF.pdf}
    \put(-20,88){\footnotesize$P_1$}
    \put(-20,20){\footnotesize$P_2$}
    \put(-160,65){\footnotesize$\mathbb{E}$}
    \put(-195,70){\footnotesize$E_j$}
    \put(-115,22){\footnotesize$\mathbb{E}$}
    \put(-39,53){\footnotesize$\goal$}
    \put(-200,15){\footnotesize$\play$}
    \caption{If $P_1$ and $P_2$ can cooperatively ensure that the enclosure region $\mathbb{E}$ containing $E_j$ never intersects with $\goal$, then the enclosure region pursuit (ERP) winning is achieved.}
    \label{fig:ERP-winning}
\end{figure}


% \begin{defi}[Interception and projection points]\label{defi:interception-point}
% Given a merged PPF $h$, if $X_{cj} \in \mathcal{C}_s^c$ and $\rho(\mathbb{E}(X_{cj};h),\goal)\ge0$, let the interception point $\bm{x}_{I} \in \mathbb{E}(X_{cj};h)$ and the projection point $\bm{x}_{G} \in \goal$ be the unique pair such that $\enVert[0]{\bm{x}_I-\bm{x}_G}_2=\rho(\mathbb{E}(X_{cj};h),\goal)$, that is, the pair $(\bm{x}_I,\bm{x}_G)$ is the unique solution of the convex problem
% \begin{equation}\label{eq:convex-pbm-IG}
% \begin{aligned}
% \mathcal{P}_{sj} : \; & \underset{(\bm{x},\bm{y})\in\mathbb{R}^2\times\mathbb{R}^2}{\textup{minimize}}
% 	&& \rho(\bm{x},\bm{y})\\
% 	&\textup{ subject to}&& f_{ij}(\bm{x},X_{ij})\ge 0,\; g(\bm{y})\le 0, \; \forall i\in s.
% \end{aligned}
% \end{equation}
% \end{defi}

% \subsection{Support constraints for convex program}

\subsection{Coalition reduction}
The convex optimization problem $\mathcal{P}(X_{cj})$ in \eqref{eq:convex-pbm-IG} is used to compute the safe distance which plays a vital role in the following analysis. Noting this, we next prove that given $X_{cj}$, there are at most two PEFs in $f_c$ which are necessary to solve $\mathcal{P}(X_{cj})$, greatly simplifying the computation. This also implies that at most two pursuers in $P_c$ work when computing $\bm{x}_I$.



% We first recall a classical result due to Helly; see \cite{RTR:15}.

% \begin{lema}[Helly]
% Let $\{\mathcal{X}_i\}_{i=1,\dots,q}$ be a finite collection of convex sets in $\mathbb{R}^n$. If every sub-collection consisting of $n+1$ sets has a nonempty intersection, then the entire collection has a nonempty intersection.
% \end{lema}

% Consider the optimization problem
% \begin{equation}\label{eq:convex-pbm-support}
% \begin{aligned}
%     \mathcal{P} : \; & \underset{\bm{x}, \bm{y} \in \mathbb{R}^n }{\textup{minimize}} & & \phi(\bm{x}, \bm{y}) \\
%     & \textup{subject to} & & \bm{x} \in \bigcap_{i \in \{1,\dots,m\}} \mathcal{X}_i, \; \bm{y} \in \mathcal{Y}
% \end{aligned}
% \end{equation}
% where $\phi(\bm{x},\bm{y})$ is a convex and continuous function in $(\bm{x}, \bm{y})$, $\mathcal{X}_i$ ($i=1,\dots,m$) and $\mathcal{Y}$ are closed convex sets such that $(\cap_{i \in \{1,\dots,m\}} \mathcal{X}_i) \cap \mathcal{Y}  = \emptyset$, and define the programs $\mathcal{P}_k$, $k=1,\dots,m$ obtained from $\mathcal{P}$ by removing the $k$th constraint
% \begin{equation*}
% \begin{aligned}
%     \mathcal{P}_k : \; & \underset{\bm{x}, \bm{y} \in \mathbb{R}^n }{\textup{minimize}} & & \phi(\bm{x}, \bm{y}) \\
%     & \textup{subject to} & & \bm{x} \in \bigcap_{i \in \{1,\dots,m\} \setminus k} \mathcal{X}_i, \; \bm{y} \in \mathcal{Y}.
% \end{aligned}
% \end{equation*}
% We assume program $\mathcal{P}$ and the programs $\mathcal{P}_k$ admit an optimal solution, say $(\bm{x}^*, \bm{y}^*)$ and $(\bm{x}^*_k, \bm{y}^*_k)$, respectively, and let $J^*=\phi(\bm{x}^*, \bm{y}^*)$ and $J^*_k=\phi(\bm{x}^*_k, \bm{y}^*_k)$. 

% \begin{defi}[Support constraint]
% The $k$th constraint $\mathcal{X}_k$ is a \emph{support constraint} (with respect to $\bm{x}$) for $\mathcal{P}$ if $J_k^*<J^*$.
% \end{defi}

% When $\phi(\bm{x})=\bm{c}^{\top}\bm{x}$ independent of $\bm{y}$, the convex optimization problem \eqref{eq:convex-pbm-support} is degenerated into the random convex problem or scenario problems which have been widely studied \cite{GCC-MCC:06,MCC-SG:08,GCC:10,AC-SG-MCC:14}. We first recall a well-known result in scenario problems due to Calafiore; see \cite{GC-MCC:05}.

% \begin{lema}[Calafiore]
% If $\phi(\bm{x})=\bm{c}^{\top}\bm{x}$, then the number of support constraints for problem $\mathcal{P}$ is at most $n$.
% \end{lema}

% % Next we prove that a similar result to the above is concluded for all convex objective functions by limiting to strictly convex constraint sets.

% We extend the above results to more general functions beyond linear functions, as well as introducing another variable of the same dimension. We start with a a technical lemma.

% % We start with a a technical lemma.

% \begin{lema}[{\cite[Lemma 1]{GC-MCC:05}}]\label{lema:p-plus-2-hyperplane}
% Given a set $Q$ of $q+2$ points in $\mathbb{R}^q$, there exist two points among these, say $\xi_1,\xi_2$, such that the line segment $\overline{\xi_1\xi_2}$ intersects the hyperplane (or one of the hyperplanes if indetermination occurs) generated by the remaining $q$ points $\xi_3, \dots, \xi_{q+2}$.
% \end{lema}

% \begin{thom}[Number of support constraints]
% The number of support constraints for problem $\mathcal{P}$ is at most $n$.
% % $f$ and $\mathcal{X}_i$, $i=1,\dots,m$ satisfy the following two properties:
% % \begin{enumerate}[label = (\roman*)]
% %     \item $\bm{x}^*$ is unique and $\bm{x}^*\in \partial (\cap_{i \in \{1,\dots,m\}} \mathcal{X}_i)$;
    
% %     \item a strict local minimum solution is a global minimum solution for the program $\mathcal{P}$ and programs $\mathcal{P}_k$, $k=1,\dots,m$;
% % \end{enumerate}
% % then  
% \end{thom}

% \begin{proof}
% We prove the conclusion by contradiction. Suppose that the problem $\mathcal{P}$ has $n_S > n$ support constraints and choose any $n+1$ constraints among these, denoted $1,\dots,n+1$. Then, there exist $n+1$ solutions (say, the first $n+1$ points) $(\bm{x}_k^*, \bm{y}_k^*)$, $(k=1,\dots,n+1)$, which are optimal solutions for $\mathcal{P}_k$. 

% Let $\eta_{\textup{min}} \coloneqq \min_{ k \in \{1, \dots, n+1\}} \left(J^* - J_k^*\right)$ be the smallest objective improvement obtained by removing a support constraint and, for some $\eta$ with $0 < \eta < \eta_{\textup{min}}$, define the hypersurface $\mathcal{H}_1 \coloneqq \{(\bm{x}, \bm{y}) \mid \phi(\bm{x}, \bm{y}) = J^* - \eta\}$. By construction, the $n+1$ points $(\bm{x}_k^*, \bm{y}_k^*)$, $(k=1,\dots,n+1)$, lie in the half-space
% \begin{equation*}
%     \mathcal{H}_2 \coloneqq \{(\bm{x}, \bm{y}) \mid \phi(\bm{x}, \bm{y}) \leq J^* - \eta\},
% \end{equation*}
% while $(\bm{x}^*, \bm{y}^*)$ lies in the half-space $\{(\bm{x}, \bm{y}) \mid \phi(\bm{x}, \bm{y}) > J^* - \eta\}$. Since $\phi$ is continuous, thus $\mathcal{H}_1$ separates $(\bm{x}_k^*, \bm{y}_k^*)$, $(k=1,\dots,n+1)$ from $(\bm{x}^*, \bm{y}^*)$. Let $(\bar{\bm{x}}_k^*, \bar{\bm{y}}_k^*)$ denote the point of intersection between $\mathcal{H}_1$ and the segment $\overline{\bm{x}^*\bm{x}^*_k}$. By convexity and construction, it follows that $\bar{\bm{x}}_k^* \in \cap_{i \in \{1, \dots, n+1\} \setminus k} \mathcal{X}_i$, $\bar{\bm{y}}_k^* \in \mathcal{Y}$, and $(\bar{\bm{x}}_k^*, \bar{\bm{y}}_k^*) \in \mathcal{H}_2$.

% Suppose that there exists an index $k$ such that $\bar{\bm{x}}_k^*$ belongs to the convex hull $\textup{co}\{\bar{\bm{x}}_1^*, \dots, \bar{\bm{x}}_{k-1}^*, \cdots, \bar{\bm{x}}_{k+1}^*, \cdots, \bar{\bm{x}}_{n+1}^*\}$. Since  $\bar{\bm{x}}_i^* \in \mathcal{X}_k$ for all $i \in \{1, \dots, n+1\} \setminus k$, then all points in $\textup{co}\{\bar{\bm{x}}_1^*, \dots, \bar{\bm{x}}_{k-1}^*, \cdots, \bar{\bm{x}}_{k+1}^*, \cdots, \bar{\bm{x}}_{n+1}^*\}$ belong to $\mathcal{X}_k$, and thus $\bar{\bm{x}}_k^* \in \mathcal{X}_k$. Since $\bar{\bm{x}}_k^* \in \cap_{i \in \{1, \dots, n+1\} \setminus k} \mathcal{X}_i$, then $\bar{\bm{x}}_k^* \in \cap_{i \in \{1, \dots, n+1\}}\mathcal{X}_i$. From this, $(\bar{\bm{x}}_k^*, \bar{\bm{y}}_k^*)$ is a feasible solution for problem $\mathcal{P}$, and has a value $\phi(\bar{\bm{x}}_k^*, \bar{\bm{y}}_k^*) = J^* - \eta < \phi(\bar{\bm{x}}^*, \bar{\bm{y}}^*)$ which contradicts with the fact that $(\bar{\bm{x}}^*, \bar{\bm{y}}^*)$ is optimal for $\mathcal{P}$.

% We consider the case in which there does not exist an $\bar{\bm{x}}_k^* \in \textup{co}\{\bar{\bm{x}}_1^*, \dots, \bar{\bm{x}}_{k-1}^*, \cdots, \bar{\bm{x}}_{k+1}^*, \cdots, \bar{\bm{x}}_{n+1}^*\}$. By \lemaref{lema:p-plus-2-hyperplane}, there exist two points, say $\bar{\bm{x}}_1^*, \bar{\bm{x}}_2^*$, such that the line segment $\overline{\bar{\bm{x}}_1^* \bar{\bm{x}}_2^*}$ intersects at least one hyperplane passing through the remaining $n -1$ points $\bar{\bm{x}}_3^*, \dots, \bar{\bm{x}}_{n+1}^*$. Let $\bar{\bm{x}}_{1,2}^*$ be the intersection point (any intersection point if more than one exists). Then there exists $\gamma \in [0, 1]$ such that $\bar{\bm{x}}_{1,2}^* = \gamma \bar{\bm{x}}_{1}^* + (1 - \gamma) \bar{\bm{x}}_{2}^*$. Define $\bar{\bm{y}}_{1,2}^* \coloneqq \gamma \bar{\bm{y}}_{1}^* + (1 - \gamma) \bar{\bm{y}}_{2}^*$. Since $\bar{\bm{x}}_{1}^*, \bar{\bm{x}}_{2}^*$ belong to $\cap_{i \in \{1, \dots, n+1\} \setminus \{1, 2\}} \mathcal{X}_i$, then so is $\bar{\bm{x}}_{1,2}^*$ by convexity. Noting that $\mathcal{Y}$ is convex, we have $\bar{\bm{y}}_{1,2}^* \in \mathcal{Y}$. The half-space $\mathcal{H}_2$ is convex as $\phi$ is a convex function, and therefore $(\bar{\bm{x}}_{1,2}^*, \bar{\bm{y}}_{1,2}^*) \in \mathcal{H}_2$. Now, $\bar{\bm{x}}_{1,2}^*, \bar{\bm{x}}_{3}^*, \dots, \bar{\bm{x}}_{n+1}^*$ are $n$ points in a flat of dimension $n -2$. Again, if one of these points belongs to the convex hull of the others, then this point satisfies all constraints, and we are done. For the remaining proofs, it follows from the same argument in the proof of \cite[Theorem 2]{GC-MCC:05}.
% \end{proof}


Instead of concentrating on the specific convex problem  \eqref{eq:convex-pbm-IG}, we consider support constraints (defined later) for more general convex optimization problems. Consider the optimization problem
\begin{equation}\label{eq:convex-pbm-support}
    \mathcal{P} : \; \underset{\bm{x}\in \mathbb{R}^n }{\textup{minimize}} \; \phi(\bm{x}) \quad \textup{subject to :} \; \bm{x} \in \bigcap_{i \in \{1,\dots,m\}} \mathcal{X}_i
\end{equation}
where $\phi(\bm{x})$ is a real-valued function in $\bm{x}$ and $\mathcal{X}_i$ ($i=1,\dots,m$) are closed convex sets. Then, define the programs $\mathcal{P}_k$, $k=1,\dots,m$ obtained from $\mathcal{P}$ by removing the $k$th constraint
\begin{equation*}
    \mathcal{P}_k : \; \underset{\bm{x}\in \mathbb{R}^n }{\textup{minimize}} \; \phi(\bm{x}) \quad \textup{subject to :} \; \bm{x} \in \bigcap_{i \in \{1,\dots,m\} \setminus k} \mathcal{X}_i.
\end{equation*}
We assume program $\mathcal{P}$ and the programs $\mathcal{P}_k$ admit an optimal solution, say $\bm{x}^*$ and $\bm{x}^*_k$, respectively, and let $J^*=\phi(\bm{x}^*)$ and $J^*_k=\phi(\bm{x}^*_k)$. 

\begin{defi}{\rm (Support constraint).}
The $k$th constraint $\mathcal{X}_k$ is a \emph{support constraint} for $\mathcal{P}$ if $J_k^*<J^*$.
\end{defi}

When $\phi(\bm{x})=\bm{c}^{\top}\bm{x}$ for a constant vector $\bm{c}$, the convex optimization problem \eqref{eq:convex-pbm-support} 
% degenerates into the convex programs or scenario programs which 
has been widely studied, e.g., \cite{GCC-MCC:06,MCC-SG:08,GCC:10,AC-SG-MCC:14}. We first recall a well-known result due to Calafiore and Campi; see \cite{GCC-MCC:06}.

\begin{lema}\label{lema:calafiore}{\rm (Calafiore and Campi).}
If $\phi(\bm{x})=\bm{c}^{\top}\bm{x}$ and program $\mathcal{P}$ and the programs $\mathcal{P}_k$ admit a unique optimal solution, then the number of support constraints for problem $\mathcal{P}$ is at most $n$.
\end{lema}

% Next we prove that a similar result to the above is concluded for all convex objective functions by limiting to strictly convex constraint sets.

Next we extend the above results to objective functions beyond linear functions.

% We start with a a technical lemma.

% \begin{lema}[{\cite[Lemma 1]{GC-MCC:05}}]\label{lema:p-plus-2-hyperplane}
% Given a set $Q$ of $q+2$ points in $\mathbb{R}^q$, there exist two points among these, say $\xi_1,\xi_2$, such that the line segment $\overline{\xi_1\xi_2}$ intersects the hyperplane (or one of the hyperplanes if indetermination occurs) generated by the remaining $q$ points $\xi_3, \dots, \xi_{q+2}$.
% \end{lema}

\begin{thom}\label{thom:number-of-support}{\rm (Number of support constraints).}
If $\phi$ and the closed convex sets $\mathcal{X}_i$, $i=1,\dots,m$ satisfy the following two properties:
\begin{enumerate}
    \item\label{itm:unique-number-support} $\bm{x}^*$ is unique;
    
    % and $\bm{x}^*\in \partial (\cap_{i \in \{1,\dots,m\}} \mathcal{X}_i)$;
    
    \item\label{itm:local-global-support} a strict local minimum solution is a global minimum solution for the program $\mathcal{P}$ and programs $\mathcal{P}_k$, $k=1,\dots,m$;
\end{enumerate}
then the number of support constraints for problem $\mathcal{P}$ is at most $n$.

Proof. \rm
We prove the theorem by contradiction. Suppose that the problem $\mathcal{P}$ has $n+1$ support constraints, indexed by $1,\dots,n+1$. For a point $\bm{x} \in \mathbb{R}^n$ and $\epsilon >0$, let $B(\bm{x}; \epsilon) \coloneqq \{ \bm{x}' \in \mathbb{R}^n \mid \|\bm{x}' - \bm{x}\|_2 < \epsilon\}$ be the neighbourhood of $\bm{x}$ with radius $\epsilon$. Since $\bm{x}^*$ is unique by assumption, then $\bm{x}^*$ is a strict local minimum point, i.e., there exists an $\epsilon_0>0$ such that $\phi(\bm{x}) > \phi(\bm{x}^*)$ for all $\bm{x} \in B(\bm{x}^*; \epsilon_0) \cap (\cap_{i \in \{1, \dots, m\}} \mathcal{X}_i)$ and $\bm{x} \neq \bm{x}^*$. 

We first prove $\bm{x}^* \in \cap_{i \in \{1, \dots, n+1\}} \partial \mathcal{X}_i$ as follows. Suppose that there exists an index (say $k$, $1 \leq k \leq n+1$) such that $\bm{x}^* \in \interior(\mathcal{X}_k)$. Thus, there exists an $\epsilon_k > 0$ such that $B(\bm{x}^*; \epsilon_k) \subset \mathcal{X}_k$. Let $\epsilon_{0,k} \coloneqq \min \{\epsilon_0, \epsilon_k\}$. Then, it follows that 
\begin{align*}
    & B(\bm{x}^*; \epsilon_{0,k}) \cap (\cap_{i \in \{1, \dots, m\} \setminus k} \mathcal{X}_i) \\
    & \qquad \qquad \qquad \subset  B(\bm{x}^*; \epsilon_0) \cap (\cap_{i \in \{1, \dots, m\}} \mathcal{X}_i).
\end{align*}
Therefore, we have $\phi(\bm{x}) > \phi(\bm{x}^*)$ for all $\bm{x} \in B(\bm{x}^*; \epsilon_{0,k}) \cap (\cap_{i \in \{1, \dots, m\} \setminus k} \mathcal{X}_i)$ and $\bm{x} \neq \bm{x}^*$, that is, $\bm{x}^*$ is a strict local minimum point for problem $\mathcal{P}_k$. Using the property \ref{itm:local-global-support}, $\bm{x}^*$ is a global minimum point for problem $\mathcal{P}_k$, i.e., $J^* = J_k^*$, which contradicts with the fact that $\mathcal{X}_k$ is a support constraint. In conclusion, $\bm{x}^* \notin \interior(\mathcal{X}_i)$ for all $i \in \{1, \dots, n+1\}$. Therefore, $\bm{x}^* \in \cap_{i \in \{1, \dots, n+1\}} \partial \mathcal{X}_i$. 

We next consider two cases depending on whether there exists $\epsilon_1 > 0$ such that $\mathcal{X}_{-k}^B$ is unique, for all $1 \leq k \leq n + 1$, where $\mathcal{X}_{-k}^B \triangleq B(\bm{x}^*; \epsilon_1) \cap (\cap_{i \in \{1, \dots, n+1\} \setminus k} \mathcal{X}_i)$.

Case 1: there exists $\epsilon_1 > 0$ such that $\mathcal{X}_{-k}^B$ is unique, i.e., $\{\bm{x}^*\}$, for all $1 \leq k \leq n + 1$. We next consider two cases depending on whether $\bm{x}^*$ is strictly minimizing $\phi$ over $\mathcal{X}^B_{-k}$. On the one hand, if there exists $k$ such that $\bm{x}^*$ is a strict minimum point over $\mathcal{X}_{-k}^B$, then considering that $\bm{x}^* \in \mathcal{X}_i$ for all $i \in \{n+2, \dots, m\}$, then $\bm{x}^*$ is also a strict minimum point over $B(\bm{x}^*; \epsilon_1) \cap (\cap_{i \in \{1, \dots, m\} \setminus k} \mathcal{X}_i)$, that is, $\bm{x}^*$ is a strict local minimum point for problem $\mathcal{P}_k$. Using the property \ref{itm:local-global-support}, $\bm{x}^*$ is a global minimum point for problem $\mathcal{P}_k$, i.e., $J^* = J_k^*$, which contradicts with the fact that $\mathcal{X}_k$ is a support constraint. 

On the other hand, if $\bm{x}^*$ is not a strict minimum point over $\mathcal{X}_{-k}^B$ for all $1 \leq k \leq n + 1$, then for each $k$, there exists a point $\overline{\bm{x}}_k \in \mathcal{X}_{-k}^B$ such that $\overline{\bm{x}}_k \neq \bm{x}^*$ and $\phi(\overline{\bm{x}}_k) \leq \phi(\bm{x}^*)$. Next, we show the contradiction by following the proof of \cite[Theorem 2]{GC-MCC:05-2}. Consider the line segments connecting $\bm{x}^*$ with each of the $\overline{\bm{x}}_k$, $1 \leq k \leq n+1$, and consider a hyperplane  

there exists a point $\bm{x}_1 \in \mathcal{X}_B$ such that
\begin{equation}\label{eq:x1-existence}
    \bm{x}_1 \neq \bm{x}^*, \, \| \bm{x}_1 - \bm{x}^* \|_2 \leq \epsilon, \, \phi(\bm{x}_1) \leq \phi(\bm{x}^*) .
\end{equation}
For \eqref{eq:x1-existence}, we take $\epsilon = \epsilon_1$. Since $B(\bm{x}^*; \epsilon_1) \cap (\cap_{i \in \{2, \dots, n+1\}} \partial\mathcal{X}_i)$ is unique (i.e., $\{ \bm{x}^* \}$), then $\bm{x}_1 \notin \cap_{i \in \{2, \dots, n+1\}} \partial\mathcal{X}_i$. Thus, there exists a set (say $\mathcal{X}_k, 2 \leq k \leq n+1$) such that $\bm{x}_1 \in \interior(\mathcal{X}_k)$

Since i) $\mathcal{X}_1$ and $\cap_{i \in \{2, \dots, n+1\}}\mathcal{X}_i$ are closed and convex, ii) $(\cap_{i \in \{2, \dots, n+1\}} \partial\mathcal{X}_i) \subset \partial (\cap_{i \in \{2, \dots, n+1\}} \mathcal{X}_i)$ and iii) $\mathcal{X}_1$ and $(\cap_{i \in \{2, \dots, n+1\}} \partial\mathcal{X}_i)$ have a unique intersection point $\bm{x}^*$ in $B(\bm{x}^*; \epsilon_1)$, then $\mathcal{X}_1$ and $\cap_{i \in \{2, \dots, n+1\}}\mathcal{X}_i$ inscribe with each other in $B(\bm{x}^*; \epsilon_1)$. Let $\bar{\epsilon}_1 \coloneqq \min\{\epsilon_1, \epsilon_0\}$. If $\mathcal{X}_1$ inscribes inside $\cap_{i \in \{2, \dots, n+1\}}\mathcal{X}_i$ within $B(\bm{x}^*; \epsilon_1)$, then
\begin{equation*}
    B(\bm{x}^*; \bar{\epsilon}_1) \cap \mathcal{X}_1 \subset B(\bm{x}^*; \bar{\epsilon}_1) \cap (\cap_{i \in \{2, \dots, n+1\}}\mathcal{X}_i). 
\end{equation*}
Intersecting with $\cap_{i \in \{1, \dots, m\} \setminus 2} \mathcal{X}_i$ for the above two sets, we have
\begin{equation*}
    B(\bm{x}^*; \bar{\epsilon}_1) \cap (\cap_{i \in \{1, \dots, m\} \setminus 2}\mathcal{X}_i) \subset B(\bm{x}^*; \epsilon_0) \cap (\cap_{i \in \{1, \dots, m\}}\mathcal{X}_i).
\end{equation*}
Thus, it follows that $\phi(\bm{x}) > \phi(\bm{x}^*)$ for all $\bm{x} \in B(\bm{x}^*; \bar{\epsilon}_1) \cap (\cap_{i \in \{1, \dots, m\} \setminus 2}\mathcal{X}_i)$ and $\bm{x} \neq \bm{x}^*$, that is, $\bm{x}^*$ is a strict local minimum point for problem $\mathcal{P}_{2}$. Using the property \ref{itm:local-global-support}, $\bm{x}^*$ is a global minimum point for problem $\mathcal{P}_2$, i.e., $J^* = J_2^*$, which contradicts with the fact that $\mathcal{X}_2$ is a support constraint. On the other side, if $\cap_{i \in \{2, \dots, n+1\}}\mathcal{X}_i$ inscribes inside $\mathcal{X}_1$ within $B(\bm{x}^*; \epsilon_1)$, then
\begin{equation*}
    B(\bm{x}^*; \bar{\epsilon}_1) \cap (\cap_{i \in \{2, \dots, n+1\}}\mathcal{X}_i) \subset B(\bm{x}^*; \bar{\epsilon}_1) \cap \mathcal{X}_1.
\end{equation*}
Intersecting with $\cap_{i \in \{1, \dots, m\} \setminus 1}\mathcal{X}_i$ for the above two sets, we have
\begin{equation*}
    B(\bm{x}^*; \bar{\epsilon}_1) \cap (\cap_{i \in \{1, \dots, m\} \setminus 1}\mathcal{X}_i) \subset B(\bm{x}^*; \epsilon_0) \cap (\cap_{i \in \{1, \dots, m\}}\mathcal{X}_i).
\end{equation*}
Thus, it follows that $\phi(\bm{x}) > \phi(\bm{x}^*)$ for all $\bm{x} \in B(\bm{x}^*; \bar{\epsilon}_1) \cap (\cap_{i \in \{1, \dots, m\} \setminus 1}\mathcal{X}_i)$ and $\bm{x} \neq \bm{x}^*$, that is, $\bm{x}^*$ is a strict local minimum point for problem $\mathcal{P}_1$, which contradicts with the fact that $\mathcal{X}_1$ is a support constraint using the same argument.

Case 2: there does not exist $\epsilon_1 > 0$ such that $B(\bm{x}^*; \epsilon_1) \cap (\cap_{i \in \{2, \dots, n+1\}} \partial\mathcal{X}_i)$ is unique. Recall $\bm{x}^* \in \cap_{i \in \{1, \dots, n+1\}} \partial \mathcal{X}_i$ and each $\partial \mathcal{X}_i$ is an $n$-dimensional hypersurface. Take two indexes from $\{2, \dots, n+1\}$, say $2$ and $3$. Suppose that $\cap_{i \in \{2, 3\}} \partial\mathcal{X}_i$ is an $n$-dimensional hypersurface in some neighbourhood of $\bm{x}^*$. Thus, $\partial \mathcal{X}_2$ and $\partial \mathcal{X}_3$ coincide in this neighbourhood. Then, there must exist an $\epsilon_{2,3} > 0$ such that $B(\bm{x}^*; \epsilon_{2,3}) \cap \mathcal{X}_2 \subset B(\bm{x}^*; \epsilon_{2,3}) \cap (\cap_{i \in \{2, 3\}} \mathcal{X}_i)$ noting that $\mathcal{X}_2, \mathcal{X}_3$ are closed convex sets. Let $\bar{\epsilon}_{2,3} \coloneqq \min\{\epsilon_0, \epsilon_{2,3}\}$. Intersecting with $\cap_{i \in \{1, 4, \dots, m\}}\mathcal{X}_i$ for the above two sets, we have  
\begin{equation*}
\begin{aligned}
     & B(\bm{x}^*; \bar{\epsilon}_{2,3}) \cap (\cap_{i \in \{1, \dots, m\} \setminus 3}\mathcal{X}_i) \\
     & \qquad \qquad \qquad  \subset B(\bm{x}^*; \epsilon_0) \cap (\cap_{i \in \{1, \dots, m\}}\mathcal{X}_i). 
\end{aligned}
\end{equation*}
Therefore, it follows that $\phi(\bm{x}) > \phi(\bm{x}^*)$ for all $\bm{x} \in B(\bm{x}^*; \bar{\epsilon}_{2,3}) \cap (\cap_{i \in \{1, \dots, m\} \setminus 3}\mathcal{X}_i)$ and $\bm{x} \neq \bm{x}^*$, that is, $\bm{x}^*$ is a strict local minimum point for problem $\mathcal{P}_3$, which similarly contradicts with the fact that $\mathcal{X}_3$ is a support constraint. Thus, $\cap_{i \in \{2, 3\}} \partial\mathcal{X}_i$ is at most $(n-1)$-dimensional in some neighbourhood of $\bm{x}^*$. We take another index (different from $2,3$) from $\{2, \dots, n+1\}$, say $4$. From the above, the hypersurface $\cap_{i \in \{2, 3, 4\}} \partial\mathcal{X}_i$ is at most $(n-1)$-dimensional in some neighbourhood of $\bm{x}^*$. Now, suppose that $\cap_{i \in \{2, 3, 4\}} \partial\mathcal{X}_i$ is  $(n-1)$-dimensional in some neighbourhood of $\bm{x}^*$. It implies that $\cap_{i \in \{2, 3\}} \partial\mathcal{X}_i$ is $(n-1)$-dimensional and thus coincides with $\partial \mathcal{X}_4$ in this neighbourhood. Then, there must exist an $\epsilon_{2,3,4} > 0$ such that $B(\bm{x}^*; \epsilon_{2,3,4}) \cap (\cap_{i \in \{2, 3\}}\mathcal{X}_i) \subset B(\bm{x}^*; \epsilon_{2, 3, 4}) \cap (\cap_{i \in \{2, 3, 4\}} \mathcal{X}_i)$ noting that $\cap_{i \in \{2, 3\}}\mathcal{X}_i, \mathcal{X}_4$ are closed convex sets. Let $\bar{\epsilon}_{2, 3, 4} \coloneqq \min\{\epsilon_0, \epsilon_{2, 3, 4}\}$. Intersecting with $\cap_{i \in \{1, 5, \dots, m\}}\mathcal{X}_i$ for the above two sets, we have 
\begin{equation*}
\begin{aligned}
     & B(\bm{x}^*; \bar{\epsilon}_{2, 3, 4}) \cap (\cap_{i \in \{1, \dots, m\} \setminus 4}\mathcal{X}_i) \\
     & \qquad \qquad \qquad \subset B(\bm{x}^*; \epsilon_0) \cap (\cap_{i \in \{1, \dots, m\}}\mathcal{X}_i)
\end{aligned}
\end{equation*}
which similarly contradicts with the fact that $\mathcal{X}_4$ is a support constraint. Thus, $\cap_{i \in \{2, 3, 4\}} \partial\mathcal{X}_i$ is at most $(n-2)$-dimensional in some neighbourhood of $\bm{x}^*$. We repeat the process until $n+1$, and determine that the hypersurface $\cap_{i \in \{2, \dots, n+1\}} \partial\mathcal{X}_i$ is at most one-dimensional in some neighbourhood of $\bm{x}^*$, i.e., $\cap_{i \in \{2, \dots, n+1\}} \partial\mathcal{X}_i = \{\bm{x}^*\}$ in some neighbourhood of $\bm{x}^*$. Therefore, we reach the contradiction that there exists $\epsilon_1 > 0$ such that $B(\bm{x}^*; \epsilon_1) \cap (\cap_{i \in \{2, \dots, n+1\}} \partial\mathcal{X}_i)$ is unique.

If $\mathcal{P}$ has $n+2$ or more support constraints, we can prove the contradiction similarly.\qed
\end{thom}

\begin{rek}
The result of Calafiore and Campi in \lemaref{lema:calafiore} is implied by \thomref{thom:number-of-support}: if the program $\mathcal{P}$ and programs $\mathcal{P}_k$, $k=1, \dots, m$, admit a unique optimal solution, then two properties \ref{itm:unique-number-support} and \ref{itm:local-global-support} in \thomref{thom:number-of-support} hold naturally due to the linearity of $\phi$. However, the objective function $\phi$ in \thomref{thom:number-of-support} need not be linear functions as used below in the context of the ERP winning.
\end{rek}

% Now we apply the results to the games considered here. 
By \thomref{thom:number-of-support}, the convex program $\mathcal{P}(X_{cj})$ in \eqref{eq:convex-pbm-IG} can be solved through a convex program with less constraints.

\begin{lema}\label{lema:constraint-reduction}{\rm (Constraint reduction).}Let $J^*_{cj}$ be the optimal value of the convex program $\mathcal{P}(X_{cj})$. Then, there exists a subcoalition $\bar{c}$ of $c$ such that $|\bar{c}| \leq 2$ and $J_{cj}^* = J^*_{\bar{c}j}$, where $J^*_{\bar{c}j}$ is the optimal value of the convex optimization problem $\mathcal{P}(X_{\bar{c}j})$:
\begin{equation}\label{eq:convex-pbm-IG-reduction}
\begin{aligned}
 & \underset{(\bm{x},\bm{y})\in\mathbb{R}^2\times\mathbb{R}^2}{\textup{minimize}}	&& d (\bm{x},\bm{y})\\
	&\textup{ subject to}&& f_i(\bm{x},X_{ij})\ge 0,\; g(\bm{y})\le 0, \; \forall i\in \bar{c}.
\end{aligned}
\end{equation}

Proof. \rm
The projection operator $\textup{Proj}_{\goal} : \mathbb{R}^2 \to \goal$ defined by $\textup{Proj}_{\goal}(\bm{x}) \coloneqq \argmin_{\bm{y} \in \goal} \|\bm{x} - \bm{y}\|_2$ computes the orthogonal projection of $\bm{x}$ onto $\goal$. It follows that $\mathcal{P}(X_{cj})$ can be rewritten as
\begin{equation}\label{eq:new-P-sj}
\begin{aligned}
& \underset{\bm{x} \in \mathbb{R}^2}{\textup{minimize}}
	&& d(\bm{x}, \textup{Proj}_{\goal}(\bm{x}))\\
	&\textup{subject to}&& \bm{x} \in \mathbb{E}(X_{ij};f_i),\; \forall i\in c.
\end{aligned}
\end{equation}
Note that $\mathbb{E}(X_{cj}; f_c)$ is closed and strictly convex, and $\goal$ is closed and convex. Then, \eqref{eq:new-P-sj} satisfies both two properties \ref{itm:unique-number-support} and \ref{itm:local-global-support} in \thomref{thom:number-of-support}, and thus has at most $2$ support constraints.\qed
\end{lema}



\section{ERP Winning State Generation}\label{sec:sink-winning-subspace}

If a set of states are known to be ERP winning, establishing the connection between this set and other states in $\mathcal{S}_{cj}$ can help to find more ERP winning states increasingly. This section proposes an \emph{steer-to-ERP} approach to verify whether a state is ERP winning based on the known ERP winning states, via steering the system to a known ERP winning state.

% In order to verify the ERP winning, this section proposes an \emph{steer-to-ERP} approach. Th
% on which the pursuit winning is guaranteed. 

% \begin{defi}{\rm (Sink winning subspace).}\label{defi:sws}
% Given a set $f_c$ of PEFs, a subspace $\mathcal{X}_{cj} \subset \mathcal{S}_{cj}$ is a \emph{sink winning subspace} of $P_c$ against $E_j$ if
% \begin{enumerate}
%     \item \label{itm:SWS-defi-1}
%     $\varrho(X_{cj}; f_c) > 0 $ for all $X_{cj} \in \mathcal{X}_{cj}$;
    
%     \item\label{itm:SWS-defi-2} there exists a pursuit strategy $U_c^{in}$ of $P_c$  defined over $\mathcal{X}_{cj}$, such that
%     $X_{cj}^t \in \mathcal{X}_{cj}$ for all $t \ge 0$ and all $X_{cj} \in \mathcal{X}_{cj}$. We call $U_c^{in}$ the \textup{in-sink strategy}.
% \end{enumerate}
% \end{defi}

% \begin{defi}[Sink winning subspace]\label{defi:sws}
% Given a set $f_c$ of PEFs, consider a subspace 
% \[\mathcal{X}_{cj} = \{ X_{cj} \in \mathcal{X}_{cj}^{\sigma} \mid \varrho(X_{cj}; f_c) \ge 0 \}\]
% where $\mathcal{X}_{cj}^{\sigma} = \{ X_{cj} \in \mathcal{S}_{cj}\mid\theta_{P_i} = \sigma_i(X_{cj}), i \in c \}$, and $\sigma_i : \mathcal{S}_{cj}\to [0, 2 \pi)$ is a heading function for $P_i (i \in c)$. If there exists a pursuit strategy $U_c$ of $P_c$ such that
% \begin{enumerate}
%     \item\label{itm:SWS-defi-1}
%     $X_{cj}^t \in \mathcal{X}_{cj}$ for all $t \ge 0$ and all $X_{cj} \in \mathcal{X}_{cj}$;
    
%     \item \label{itm:SWS-defi-2} there exists a finite horizon $T \ge 0$ such that for $X_{cj} \in \mathcal{S}_{cj}$, then $X_{cj}^t \in \mathcal{X}_{cj}^{\sigma}$ for some $0 \leq t \leq T$.
% \end{enumerate}
% then $\mathcal{X}_{cj}$ is a \emph{sink winning subspace} and $U_c$ is a \textup{sink strategy}.
% \end{defi}

% \subsection{Pursuit strategies and parameters for one pursuer}\label{subsec:strategy-one-pursuer}

% This definition shows that all states in the sink winning subspace are ERP winning states. We next adopt it to verify that a state is the ERP winning. 
% To simplify the notation, we assume a pursuer $P \in \pteam $ with a PEF $f$ and its absorbing function $\sigma$, capture radius $r > 0$ and minimum turning radius $\kappa > 0$, as well as its speed ratio $\alpha > 1$ over an evader $E \in \eteam$. Then, the system state for $P$ and $E$ is denoted by $X = (\bm{x}_P, \theta_P, \bm{x}_E) \in \mathcal{A}_1$, where $\mathcal{A}_1$ is the states with non-negative safe distance under $f$. 
The following notations will be required. For a PEF $f_i$, we define $f_{i, \bm{x}}(\bm{x}, X_{ij}) = \partial f (\bm{x}, X_{ij})/ \partial \bm{x}$, $f_{i, P}(\bm{x}, X_{ij}) = \partial f (\bm{x}, X_{ij})/ \partial \bm{x}_{P_i}$, $f_{i, \theta}(\bm{x}, X_{ij}) = \partial f (\bm{x}, X_{ij}) / \partial \theta_{P_i} $, and $f_{i, E}(\bm{x}, X_{ij}) = \partial f (\bm{x}, X_{ij}) / \partial \bm{x}_{E_j} $. For two distinct points $\bm{x} \in \mathbb{R}^2 $ and $\bm{y} \in \mathbb{R}^2$, let $d_{\bm{x}} (\bm{x}, \bm{y}) = \partial d (\bm{x}, \bm{y}) / \partial \bm{x}$ and $d_{\bm{y}} (\bm{x}, \bm{y}) = \partial d (\bm{x}, \bm{y}) / \partial \bm{y}$. Let $\bm{e}_{\theta_{P_i}} = [\cos \theta_{P_i}, \sin \theta_{P_i}]^\top$.


% Let $\bar{f}_{\bm{y}}(\bm{x}, \bm{y}, \theta, \bm{z}) = \pdirect^{\top} f_{\bm{y}}(\bm{x}, \bm{y}, \theta, \bm{z})$. We define the derivatives for $f^{\sigma}$ similarly. 

% For any $\theta \in \mathbb{R}$, let $\bm{e}_{\theta^{\perp}} = [- \sin \theta, \cos \theta]^{\top} \in \partial\mathbb{S}^2$.

% Unless for clarity, the subscripts $i$ and $j$ are omitted in this section. 

% Thus, we denote the notation $\alpha_{ij}$, $\kappa_i$, $r_i$, $v_{P_i}$, $v_{E_j}$, $f_i$, $X_{ij}$, $\mathcal{A}_{ij}$, $\eta_{ij}$ by $\alpha$, $\kappa$, $r$, $v_{P}$, $v_{E}$, $f$, $X$, $\mathcal{A}_1$ and $\eta$, respectively. 



% there exists a pursuit strategy $u_{P}(\cdot)$ such that $\od{}{t}{\varrho}(X, f) \ge 0$ for all $X \in \mathcal{X}$, regardless of $\bm{u}_E$, 
\begin{thom}\label{thom:nece-suff-no-closing-nv1}{\rm (Steer-to-ERP approach).} 
Given a set $f_c$ of PEFs and a state $X_{cj} \in \mathcal{S}_{cj}$, if there exists a pursuit strategy $U_c^1$ of $P_c$ and a time horizon $T \in \mathbb{R}_{\ge 0}$ such that $X_{cj}^t$ is an ERP winning state for some $t \in [0, T]$ regardless of $\bm{u}_{E_j}$, and $\varrho(X_{cj}; f_c) > \max \{-V T, 0\} $, where $V$ is the optimal value of problem
\begin{equation}\label{eq:optimization-pbm-set-nv1}
    \begin{aligned}
       & \textup{minimize} & &  \sum\nolimits_{i \in c}  v_{P_i} \lambda_i \big ( f_{i,P}^\top \bm{e}_{\theta_{P_i}} + \frac{  |f_{i,\theta}| }{\kappa_i } + \frac{\| f_{i,E} \|_2}{\alpha_{ij}} \big) \\
       & \textup{variables}&& \bm{x}_I \in \mathbb{R}^2 ,\bm{x}_G \in \mathbb{R}^2, X'_{cj} \in \mathcal{S}_{cj}, \lambda_i, \lambda_g, i \in c \\
       &\textup{subject to} & & \bm{0}= \lambda_g g_{\bm{y}}(\bm{x}_G)  + \sum\nolimits_{i \in c} \lambda_i f_{i, \bm{x}} (\bm{x}_I, X'_{ij} ) \\
       & & & \bm{0}= d_{\bm{y}} ( \bm{x}_I, \bm{x}_G) + \lambda_g g_{\bm{y}}(\bm{x}_G), \forall \bm{x}_I \neq \bm{x}_G \\
       & & & f_i ( \bm{x}_I, X'_{ij}) \ge 0, \lambda_i \leq 0, \lambda_i f_i ( \bm{x}_I, X'_{ij}) = 0 \\
       & & &  i \in c, g(\bm{x}_G) = 0,  \lambda_g \ge 0
    \end{aligned}
\end{equation}
then $X_{cj}$ is an ERP winning state. Moreover, if $U_c^2$ is an ERP winning strategy for $X_{cj}^t$, then adopting $U_c^1$ for $[0, t]$ and $U_c^2$ for $(t, \infty)$ is an ERP winning strategy for $X_{cj}$.

% Given a set $f_c$ of PEFs, let $\mathcal{X}_{cj}$ be a sink winning subspace with an in-sink straetgy $U_c^{in}$. For a state $X_{cj} \in \mathcal{S}_{cj}$, if there exists a pursuit strategy $U_c^{out}$ of $P_c$ defined over $\mathcal{S}_{cj}\setminus \mathcal{X}_{cj}$ and a time horizon $T \in \mathbb{R}_{\ge 0}$ such that $X_{cj}^t \in \mathcal{X}_{cj}$ for some $t \in [0, T]$ regardless of $\bm{u}_{E_j}$ and $\varrho(X_{cj}; f_c) > \max \{-V T, 0\} $, where $V$ is the optimal value of problem
% \begin{equation}\label{eq:optimization-pbm-set-nv1}
%     \begin{aligned}
%        & \textup{minimize} & &  \sum\nolimits_{i \in c}  \lambda_i ( f_{i,P}^\top \dot{\bm{x}}_{P_i} + \frac{|f_{i,\theta}| v_{P_i}}{\kappa_i } + v_{E_j} \| f_{i,E} \|_2) \\
%        & \textup{variables}&& \bm{x}_I \in \mathbb{R}^2 ,\bm{x}_G \in \mathbb{R}^2, X'_{cj} \in \mathcal{S}_{cj}, \lambda_i, \lambda_g, i \in c \\
%        &\textup{subject to} & & \bm{0}= \lambda_g g_{\bm{y}}(\bm{x}_G)  + \sum\nolimits_{i \in c} \lambda_i f_{i, \bm{x}} (\bm{x}_I, X'_{ij} ) \\
%        & & & \bm{0}= d_{\bm{y}} ( \bm{x}_I, \bm{x}_G) + \lambda_g g_{\bm{y}}(\bm{x}_G), \forall \bm{x}_I \neq \bm{x}_G \\
%        & & & f_i ( \bm{x}_I, X'_{ij}) \ge 0, \lambda_i \leq 0, \lambda_i f_i ( \bm{x}_I, X'_{ij}) = 0 \\
%        & & &  i \in c, g(\bm{x}_G) = 0,  \lambda_g \ge 0
%     \end{aligned}
% \end{equation}
% \begin{equation}\label{eq:optimization-pbm}
%     \begin{aligned}
%       & \textup{maximize} & & \alpha \kappa \bar{f}_{P}(\bm{x}, X) - \alpha  \left |f_{\theta}(\bm{x}, X) \right| + \kappa \left\|f_{E}(\bm{x}, X) \right\|_2 \\
%       & \textup{variables}&& \bm{x} \in \mathbb{R}^2, \bm{y} \in \mathbb{R}^2, X \in \mathcal{X} \cap \mathcal{C}_N, \xi_1, \xi_2 \in \mathbb{R}_{> 0} \\
%       &\textup{subject to} & & f(\bm{x}, X) = 0, g(\bm{y}) = 0, f_{\bm{x}}(\bm{x}, X) = \xi_1 g_{\bm{y}}(\bm{y}), \\
%       & & & \bm{x} - \bm{y} = \xi_2 \left \|\bm{x} - \bm{y} \right \|_2 g_{\bm{y}}(\bm{y}),
%     \end{aligned}
% \end{equation}
% then $X_{cj}$ is an ERP winning state. Moreover, the strategy $(U_c^{in}, U_c^{out})$ is an ERP winning strategy.

% Given a set of states $\mathcal{X} \subset \mathcal{A}_1$, $P$ achieves no-approaching winning against $E$ over $\mathcal{X}$, if $V_{\mathcal{X}}^* = \max\{ V_{N}^{*}, V_{U}^{*}\} \leq 0$, where $V_{N}^{*}$ is the optimal value of the problem in the non-singular subspace $\mathcal{X} \cap \mathcal{C}_N$:
% \begin{equation}\label{eq:optimization-pbm-set-1v1}
%     \begin{aligned}
%       & \textup{maximize} & & \alpha \kappa \bar{f}_{P}(\bm{x}, X) - \alpha  \left |f_{\theta}(\bm{x}, X) \right| + \kappa \left\|f_{E}(\bm{x}, X) \right\|_2 \\
%       & \textup{variables}&& \bm{x} \in \mathbb{R}^2, \bm{y} \in \mathbb{R}^2, X \in \mathcal{X} \cap \mathcal{C}_N, \xi_1, \xi_2 \in \mathbb{R}_{> 0} \\
%       &\textup{subject to} & & f(\bm{x}, X) = 0, g(\bm{y}) = 0, f_{\bm{x}}(\bm{x}, X) = \xi_1 g_{\bm{y}}(\bm{y}), \\
%       & & & \bm{x} - \bm{y} = \xi_2 \left \|\bm{x} - \bm{y} \right \|_2 g_{\bm{y}}(\bm{y}),
%     \end{aligned}
% \end{equation}
% and $V_{U}^{*}$ is the optimal value of the problem in the universal subspace $\mathcal{X} \cap \mathcal{C}_U$:
% \begin{equation}\label{eq:optimization-pbm-set-absorb-1v1}
%     \begin{aligned}
%       & \textup{maximize} & & \alpha \bar{f}_{P}^{u}(\bm{x}, \bm{x}_P, \bm{x}_E) + \left\|f^{u}_{E}(\bm{x}, \bm{x}_P, \bm{x}_E) \right\|_2 \\
%       & \textup{variables}&& \bm{x} \in \mathbb{R}^2, \bm{y} \in \mathbb{R}^2, \xi_1, \xi_2 \in \mathbb{R}_{> 0} \\
%       & & & (\bm{x}_P, \sigma^u(\bm{x}_P, \bm{x}_E), \bm{x}_E) \in \mathcal{X} \cap \mathcal{C}_U  \\
%       &\textup{subject to} & & f^{u}(\bm{x}, \bm{x}_P, \bm{x}_E) = 0, \; g(\bm{y}) = 0, \\
%         & & & f^{u}_{\bm{x}}(\bm{x}, \bm{x}_P, \bm{x}_E) = \xi_1 g_{\bm{y}}(\bm{y}), \\
%       & & & \bm{x} - \bm{y} = \xi_2 \left \|\bm{x} - \bm{y} \right \|_2 g_{\bm{y}}(\bm{y}).
%     \end{aligned}
% \end{equation}
% If $V_{\mathcal{X}}^* \leq 0$, then the pursuit strategy $u_P(X)$ given by $-\textup{sgn}(f_{\theta}(\eta(X), X))$ if $X \in \mathcal{X} \cap \mathcal{C}_N$, $\pm 1$ if $X \in \mathcal{X} \cap \mathcal{C}_D$ and 
% \begin{equation}\label{eq:pursuit-strategy-1v1}
%      - \kappa \bm{e}_{\theta_P}^{\top} R_{90} \big( \pd{\sigma^u}{\bm{x}_P}  \bm{e}_{\theta_P} + \frac{1}{\alpha}   \pd{\sigma^u}{\bm{x}_E} \bm{u}_E \big)
%     \end{equation}
% if $X \in \mathcal{X} \cap \mathcal{C}_U $,
% is a no-approaching winning strategy.
% Consider a pursuer $P$ with a PEF $f$ and an evader $E$. 
% Given a set of states $\mathcal{X} \subset \mathcal{A}_1$, $P$ achieves no-approaching winning against $E$ over $\mathcal{X}$, if $V_{\mathcal{X}}^* = \max\{ V_{N}^{*}, V_{U}^{*}\} \leq 0$, where $V_{N}^{*}$ is the optimal value of the problem in the non-singular subspace $\mathcal{X} \cap \mathcal{C}_N$:
% \begin{equation}\label{eq:optimization-pbm-set-1v1}
%     \begin{aligned}
%       & \textup{maximize} & & \alpha \kappa \bar{f}_{P}(\bm{x}, X) - \alpha  \left |f_{\theta}(\bm{x}, X) \right| + \kappa \left\|f_{E}(\bm{x}, X) \right\|_2 \\
%       & \textup{variables}&& \bm{x} \in \mathbb{R}^2, \bm{y} \in \mathbb{R}^2, X \in \mathcal{X} \cap \mathcal{C}_N, \xi_1, \xi_2 \in \mathbb{R}_{> 0} \\
%       &\textup{subject to} & & f(\bm{x}, X) = 0, g(\bm{y}) = 0, f_{\bm{x}}(\bm{x}, X) = \xi_1 g_{\bm{y}}(\bm{y}), \\
%       & & & \bm{x} - \bm{y} = \xi_2 \left \|\bm{x} - \bm{y} \right \|_2 g_{\bm{y}}(\bm{y}),
%     \end{aligned}
% \end{equation}
% and $V_{U}^{*}$ is the optimal value of the problem in the universal subspace $\mathcal{X} \cap \mathcal{C}_U$:
% \begin{equation}\label{eq:optimization-pbm-set-absorb-1v1}
%     \begin{aligned}
%       & \textup{maximize} & & \alpha \bar{f}_{P}^{u}(\bm{x}, \bm{x}_P, \bm{x}_E) + \left\|f^{u}_{E}(\bm{x}, \bm{x}_P, \bm{x}_E) \right\|_2 \\
%       & \textup{variables}&& \bm{x} \in \mathbb{R}^2, \bm{y} \in \mathbb{R}^2, \xi_1, \xi_2 \in \mathbb{R}_{> 0} \\
%       & & & (\bm{x}_P, \sigma^u(\bm{x}_P, \bm{x}_E), \bm{x}_E) \in \mathcal{X} \cap \mathcal{C}_U  \\
%       &\textup{subject to} & & f^{u}(\bm{x}, \bm{x}_P, \bm{x}_E) = 0, \; g(\bm{y}) = 0, \\
%         & & & f^{u}_{\bm{x}}(\bm{x}, \bm{x}_P, \bm{x}_E) = \xi_1 g_{\bm{y}}(\bm{y}), \\
%       & & & \bm{x} - \bm{y} = \xi_2 \left \|\bm{x} - \bm{y} \right \|_2 g_{\bm{y}}(\bm{y}).
%     \end{aligned}
% \end{equation}
% If $V_{\mathcal{X}}^* \leq 0$, then the pursuit strategy $u_P(X)$ given by $-\textup{sgn}(f_{\theta}(\eta(X), X))$ if $X \in \mathcal{X} \cap \mathcal{C}_N$, $\pm 1$ if $X \in \mathcal{X} \cap \mathcal{C}_D$ and 
% \begin{equation}\label{eq:pursuit-strategy-1v1}
%      - \kappa \bm{e}_{\theta_P}^{\top} R_{90} \big( \pd{\sigma^u}{\bm{x}_P}  \bm{e}_{\theta_P} + \frac{1}{\alpha}   \pd{\sigma^u}{\bm{x}_E} \bm{u}_E \big)
%     \end{equation}
% if $X \in \mathcal{X} \cap \mathcal{C}_U $,
% is a no-approaching winning strategy.

Proof. \rm
Consider a state $X'_{cj} \in \mathcal{S}_{cj}$ such that $\varrho(X'_{cj}; f_c) > 0$, that is, $d (\mathbb{E}(X'_{cj}; f_c), \goal) > 0$. Since $\mathbb{E}(X'_{cj}; f_c)$ is strictly convex and $\goal$ is convex, there exists a unique solution $(\bm{x}_I, \bm{x}_G) \in \mathbb{E}(X'_{cj}; f_c) \times \goal$ to $\mathcal{P}(X'_{cj})$ in \eqref{eq:convex-pbm-IG}.

Case 1: $\bm{x}_I \neq \bm{x}_G$. By \emph{Karush-Kuhn-Tucker (KKT) conditions}, the solution $(\bm{x}_I, \bm{x}_G)$ satisfies
\begin{subequations}\label{eq:kkt-condition-nv1}
\begin{align}
	&\bm{0}= d_{\bm{x}} (\bm{x}_I, \bm{x}_G) + \sum\nolimits_{i \in c} \lambda_i f_{i, \bm{x}} (\bm{x}_I, X'_{ij}) \label{itm:winning-KKT-1}\\
	&\bm{0}= d_{\bm{y}} (\bm{x}_I, \bm{x}_G) + \lambda_g g_{\bm{y}}(\bm{x}_G) \label{itm:winning-KKT-2}\\
	& f_i (\bm{x}_I, X'_{ij}) \ge 0, \ \lambda_i \leq 0, \ \lambda_i f_i(\bm{x}_I, X'_{ij}) = 0,  \ i \in c \label{itm:winning-KKT-3}\\
	& g(\bm{x}_G)\le 0, \ \lambda_g g(\bm{x}_G) = 0, \ \lambda_g \ge 0 \label{itm:winning-KKT-4}
\end{align}
\end{subequations}
where $X'_{ij}$ is a part of $X'_{cj}$ corresponding to $P_i$, and $\lambda_i$ and $ \lambda_g$ are the Lagrange multipliers. The slackness condition \eqref{itm:winning-KKT-3} implies that the index set $c$ can be classified into two disjoint index sets $c^{=0}$ and $c^{>0}$ ($c^{>0}$ may be empty) where
\begin{equation}\label{eq:slack-condition}
\begin{cases}
f_i(\bm{x}_I, X'_{ij}) = 0, \ \lambda_i \leq 0, \quad \textup{if } i \in c^{=0} \\
f_i(\bm{x}_I, X'_{ij}) > 0, \ \lambda_i = 0, \quad \textup{if } i \in c^{>0}.
\end{cases}
\end{equation} 
Then, the enclosure region $\mathbb{E}(X'_{cj}; f_c)$ moves away from $\goal$ with the speed $\od{}{t}{\varrho} (X'_{cj}; f_c)$ that equals
\begin{equation}\label{eq:varrho-to-f-nv1}
\begin{aligned}
	 & \dod{}{t}d ( \bm{x}_I, \bm{x}_G ) =  d_{\bm{x}}^{\top}( \bm{x}_I, \bm{x}_G ) \dot{\bm{x}}_I + d_{\bm{y}}^{\top} ( \bm{x}_I, \bm{x}_G ) \dot{\bm{x}}_G \\
	& = - \sum\nolimits_{i \in c} \lambda_i f^{\top}_{i, \bm{x}} (\bm{x}_I, X'_{ij} ) \dot{\bm{x}}_I - \lambda_g g_{\bm{y}}^{\top} (\bm{x}_G ) \dot{\bm{x}}_G \\
	& = - \sum\nolimits_{i \in c} \lambda_i f^{\top}_{i, \bm{x}} (\bm{x}_I, X'_{ij} ) \dot{\bm{x}}_I
\end{aligned}
\end{equation}
where 
% the first equality follows because $\bm{x}_I$ and $\bm{x}_G$ are time-dependent, as they are computed by $X'_{cj}$ through \eqref{eq:convex-pbm-IG} which depends on $t$ due to the dynamics \eqref{eq:pursuer_car} and \eqref{eq:evader_simple}, 
the second equality follows from \eqref{eq:kkt-condition-nv1}, and the third equality follows noting $\bm{x}_G$ is always at the boundary of $\goal$, i.e., $g(\bm{x}_G) \equiv 0$ and thus $g_{\bm{y}}^{\top} (\bm{x}_G) \dot{\bm{x}}_G = 0$. For any $i \in c^{=0}$, since $\bm{x}_I$ is always at the boundary of $\mathbb{E}(X'_{ij}; f_i)$, then $f_i(\bm{x}_I, X'_{ij}) \equiv 0$,  and according to the condition \ref{itm:PEF-defi-2} in \defiref{defi:PEF}, $f_i$ is differentiable in $\bm{x}$, $\bm{x}_{P_i}$, $\theta_{P_i}$ and $\bm{x}_{E_j}$. Then, we have $\od{}{t}f_i(\bm{x}_I, X'_{ij})=0$, implying that
\begin{equation}\label{eq:f-to-control-nv1}
\begin{aligned}
& f_{i,\bm{x}}^\top (\bm{x}_I, X'_{ij}) \dot{\bm{x}}_I  = - f_{i,P}^\top \dot{\bm{x}}_{P_i} - f_{i,\theta} \dot{\theta}_{P_i} - f_{i,E}^\top  \dot{\bm{x}}_{E_j}\\
& = - v_{P_i} f_{i,P}^\top \bm{e}_{\theta_{P_i}} - f_{i,\theta} v_{P_i} u_{P_i} / \kappa_i - v_{E_j} f_{i,E}^\top  \bm{u}_{E_j}
% & = v_{E_j} ( \alpha_i \bar{f}_{i,P} (\hat{\bm{x}}, Y_{ij}) + \frac{  \alpha_i  }{\kappa_i} f_{i,\theta}(\hat{\bm{x}}, Y_{ij})u_{P_i} + f_{i,E}^\top (\hat{\bm{x}}, Y_{ij}) \bm{u}_{E_j} )
\end{aligned}
\end{equation}
where the second equality follows from \eqref{eq:pursuer_car} and \eqref{eq:evader_simple}. 

% Let $X= (\bm{x}_P, \theta_P, \bm{x}_E) \in \mathcal{X}$. Since $\mathcal{X} \subset \mathcal{A}_1$, then $\varrho(X; f)\ge0$, i.e., $\rho(\mathbb{E}(X; f), \goal) \ge 0$. Since $\mathbb{E}(X; f)$ is strictly convex and $\goal$ is convex, there exists a unique solution $(\hat{\bm{x}},\hat{\bm{y}}) \in \mathbb{E}(X; f) \times \goal$ to $\mathcal{P}(X)$ in \eqref{eq:convex-pbm-IG}. 

% Case 1: $\hat{\bm{x}} \neq \hat{\bm{y}}$. By \emph{Karush-Kuhn-Tucker (KKT) conditions}, the solution $\left(\hat{\bm{x}}, \hat{\bm{y}} \right)$ satisfies
% \begin{equation}\label{eq:kkt-condition-1v1}
% \begin{aligned}
% 	&\bm{0}= \rho_{\bm{x}} \left(\hat{\bm{x}}, \hat{\bm{y}} \right) + \lambda_1 f_{\bm{x}} \left(\hat{\bm{x}}, X \right),\\
% 	&\bm{0}= \rho_{\bm{y}} \left( \hat{\bm{x}}, \hat{\bm{y}} \right) + \lambda_2 g_{\bm{y}}(\hat{\bm{y}}),\\
% 	& f\left( \hat{\bm{x}}, X \right) \ge 0, \ g\left(\hat{\bm{y}}\right)\le 0,\ \lambda_1 \leq 0, \ \lambda_2 \ge 0, \\
% 	& \lambda_1 f\left(\hat{\bm{x}}, X \right) = 0, \ \lambda_2 g\left(\hat{\bm{y}} \right) = 0,
% \end{aligned}
% \end{equation}
% where $\lambda_1, \lambda_2\in\mathbb{R}$ are the Lagrange multipliers. Then,
% \begin{equation}\label{eq:varrho-to-f-1v1}
% \begin{aligned}
% 	 \dod{}{t}{\varrho}(X; f) & =  \dod{}{t}\rho\left( \hat{\bm{x}},\hat{\bm{y}} \right) =  \rho_{\bm{x}}^{\top}(\hat{\bm{x}}, \hat{\bm{y}}) \dod{\hat{\bm{x}}}{t} + \rho_{\bm{y}}^{\top}(\hat{\bm{x}}, \hat{\bm{y}}) \dod{\hat{\bm{y}}}{t}\\
% 	& =  - \lambda_1 f_{\bm{x}}^{\top} \left(\hat{\bm{x}}, X \right) \dod{\hat{\bm{x}}}{t} - \lambda_2 g_{\bm{y}}^{\top} (\hat{\bm{y}}) \dod{\hat{\bm{y}}}{t} \\
% 	& = - \lambda_1 f_{\bm{x}}^{\top} \left(\hat{\bm{x}}, X \right) \dod{\hat{\bm{x}}}{t},
% \end{aligned}
% \end{equation}
% where the second equality follows because $\hat{\bm{x}}$ and $\hat{\bm{y}}$ are both time-dependent, as they are computed by $X$ which depends on $t$ due to the dynamics \eqref{eq:pursuer_car} and \eqref{eq:evader_simple}, the third equality follows from \eqref{eq:kkt-condition-1v1}, and the fourth equality follows noting $\hat{\bm{y}}$ is always at the boundary of $\goal$, i.e., $g(\hat{\bm{y}}) \equiv 0$ and thus $g_{\bm{y}}^{\top} (\hat{\bm{y}}) \od{\hat{\bm{y}}}{t} = 0$. 

% Let $\mathcal{X}_N \triangleq \mathcal{X} \cap \mathcal{C}_N$. We first consider $X$ in the no-singular subspace $\mathcal{X}_N$.





% If $P_c$ aims to drive $\mathbb{E}(X_{cj}; f_c)$ away from $\goal$ with the maximum speed, i.e., minimize $-\od{}{t}{\varrho} (Y_{sj}; f_c)$, while $E_j$ seeks the opposite, then the maximum speed $V^{SW}(Y_{sj})$ of $\mathbb{E}(Y_{sj}; f_c)$ approaching $\goal$ at $Y_{sj}$ is
% Before the system state reaches the sink winning subspace $\mathcal{X}_{cj}$ under the strategy $U_c^{out}$, 

The minimum speed $V(X'_{cj})$ of $\mathbb{E}(X'_{cj}; f_c)$ moving away from $\goal$ is equal to
\begin{equation*} 
\begin{aligned}
% \label{eq:max-min-partial-rho-nv1}
& \min_{U_c \in \mathbb{U}_c} \min_{\bm{u}_{E_j} \in \mathbb{U}_E}  \dod{}{t}{\varrho}(X'_{cj}; f_c) \\ 
     % & \min_{U_c \in \mathbb{U}_c} \min_{\bm{u}_{E_j} \in \mathbb{U}_E} \sum\nolimits_{i \in c} \lambda_i ( f_{i,P}^\top \dot{\bm{x}}_{P_i} + f_{i,\theta} v_{P_i} u_{P_i} / \kappa_i + v_{E_j} f_{i,E}^\top  \bm{u}_{E_j}  )\\
     &  = \sum\nolimits_{i \in c}  \lambda_i ( v_{P_i} f_{i,P}^\top \bm{e}_{\theta_{P_i}} + |f_{i,\theta}| v_{P_i} / \kappa_i + v_{E_j} \| f_{i,E} \|_2)
\end{aligned}    
\end{equation*}
where \eqref{eq:varrho-to-f-nv1}, \eqref{eq:f-to-control-nv1} and $\lambda_i \leq 0$ are used. The constraint \eqref{eq:kkt-condition-nv1} is written as \eqref{eq:optimization-pbm-set-nv1} using $d_{\bm{x}} (\bm{x}_I, \bm{x}_G) = - d_{\bm{y}} (\bm{x}_I, \bm{x}_G)$. 
% By considering different index sets in \eqref{eq:slack-condition} and noting $\bm{x}_G$ is always at the boundary of $\goal$, the constraints \eqref{eq:kkt-condition-nv1} are simplified to
% \begin{equation*}
% \begin{aligned}
% 	&\bm{0}= \rho_{\bm{x}} (\bm{x}_I, \bm{x}_G) + \sum\nolimits_{i \in c^{=0}} \lambda_i f_{i, \bm{x}} (\bm{x}_I, X'_{ij})\\
% 	&\bm{0}= \rho_{\bm{y}} (\bm{x}_I, \bm{x}_G) + \lambda_g g_{\bm{y}}(\bm{x}_G)\\
% 	& f_i (\bm{x}_I, X'_{ij}) = 0, \ \lambda_i \leq 0, \ i \in c^{=0}\\
% 	& f_i (\bm{x}_I, X'_{ij}) > 0, \ \lambda_i = 0, \ i \in c^{>0}, \ g(\bm{x}_G) = 0, \ \lambda_g > 0.
% \end{aligned}
% \end{equation*}
Thus, the minimum speed of the enclosure region moving away from $\goal$ over $\mathcal{S}_{cj}$ is $V = \min_{X'_{cj} \in \mathcal{S}_{cj}} V(X'_{cj})$. Moreover, by assumption $P_c$ can steer the system state $X_{cj}$ to an ERP winning state $X_{cj}^t$ within the time period $T$ by using the strategy $U_c^1$.
% and force the system state to stay in $\mathcal{X}_{cj}$ by using the strategy $U_c^{in}$. 
Therefore, if the current system state $X_{cj} \in \mathcal{S}_{cj}$ is such that $\varrho(X_{cj}; f_c) > \max \{-VT, 0\} $, then the safe distance is kept before $P_c$ steers the system state to $X_{cj}^t$. Thus by \defiref{defi:ERP-winning}, $X_{cj}$ is an ERP winning state. If $U_c^2$ is an ERP winning strategy for $X_{cj}^t$, the strategy pair $(U_c^1, U_c^2)$ can form an ERP winning strategy for $X_{cj}$ as described in the conclusion.

% from which we have
% \begin{equation}\label{eq:min-f-nv1}
% \begin{aligned}
%      0 & \leq \max_{u_P \in \mathbb{U}_P} \min_{\bm{u}_E \in \mathbb{U}_E, X \in \mathcal{X}_N} - \lambda_1 f_{\bm{x}}^{\top} \left(\hat{\bm{x}}, X \right) \dod{\hat{\bm{x}}}{t}   \\
%      & = \max_{u_P \in \mathbb{U}_P} \min_{\bm{u}_E \in \mathbb{U}_E, X \in \mathcal{X}_N} \frac{\lambda_1 v_E}{\kappa} \big( \alpha \kappa \bar{f}_{P} (\hat{\bm{x}}, X)  \\
%      & \qquad \qquad  + \alpha f_{\theta}(\hat{\bm{x}}, X) u_P + \kappa f_{E}^\top (\hat{\bm{x}}, X) \bm{u}_E \big) \\
%      & = \min_{X \in \mathcal{X}_N} \frac{\lambda_1 v_E}{\kappa} \big( \alpha \kappa \bar{f}_{P} (\hat{\bm{x}}, X) - \alpha \left |f_{\theta}(\hat{\bm{x}}, X) \right| \\
%      & \qquad \quad \ + \kappa \left\| f_{E}(\hat{\bm{x}}, X) \right\|_2 \big),
% \end{aligned}
% \end{equation}

% By assumption, there exists a pursuit strategy $u_{P}$ such that $\od{}{t}{\varrho}(X; f) \ge 0$ for all $X \in \mathcal{X}_N$, regardless of $\bm{u}_E$. Equivalently, this implies that
% \begin{equation} \label{eq:max-min-partial-rho-1v1}
%     \max_{u_P \in \mathbb{U}_P} \min_{\bm{u}_E \in \mathbb{U}_E, X \in \mathcal{X}_N} \dod{}{t}{\varrho}(X; f) \ge 0,
% \end{equation}
% from which we have
% \begin{equation}\label{eq:min-f-1v1}
% \begin{aligned}
%      0 & \leq \max_{u_P \in \mathbb{U}_P} \min_{\bm{u}_E \in \mathbb{U}_E, X \in \mathcal{X}_N} - \lambda_1 f_{\bm{x}}^{\top} \left(\hat{\bm{x}}, X \right) \dod{\hat{\bm{x}}}{t}   \\
%      & = \max_{u_P \in \mathbb{U}_P} \min_{\bm{u}_E \in \mathbb{U}_E, X \in \mathcal{X}_N} \frac{\lambda_1 v_E}{\kappa} \big( \alpha \kappa \bar{f}_{P} (\hat{\bm{x}}, X)  \\
%      & \qquad \qquad  + \alpha f_{\theta}(\hat{\bm{x}}, X) u_P + \kappa f_{E}^\top (\hat{\bm{x}}, X) \bm{u}_E \big) \\
%      & = \min_{X \in \mathcal{X}_N} \frac{\lambda_1 v_E}{\kappa} \big( \alpha \kappa \bar{f}_{P} (\hat{\bm{x}}, X) - \alpha \left |f_{\theta}(\hat{\bm{x}}, X) \right| \\
%      & \qquad \quad \ + \kappa \left\| f_{E}(\hat{\bm{x}}, X) \right\|_2 \big),
% \end{aligned}
% \end{equation}
% where the first inequality follows using \eqref{eq:varrho-to-f-1v1}, the first equality is due to \eqref{eq:f-to-control-1v1}, and $\lambda_1 \leq 0$ is used in the second equality. Again, by $\lambda_1 \leq 0$, \eqref{eq:min-f-1v1} is simplified to
% \begin{equation}\label{eq:simplified-f-max-1v1}
%     \max_{X \in \mathcal{X}_N} \alpha \kappa \bar{f}_{P} (\hat{\bm{x}}, X) - \alpha \left |f_{\theta}(\hat{\bm{x}}, X) \right| + \kappa \left\| f_{E}(\hat{\bm{x}}, X) \right\|_2 \leq 0.
% \end{equation}
% Since $f(\hat{\bm{x}}, X) = 0$, $g(\hat{\bm{y}}) = 0$, $\rho_{\bm{x}} (\hat{\bm{x}}, \hat{\bm{y}}) = - \rho_{\bm{y}} (\hat{\bm{x}}, \hat{\bm{y}})$ and $\hat{\bm{x}} \neq \hat{\bm{y}}$, \eqref{eq:kkt-condition-1v1} is equivalent to
% \begin{equation}\label{eq:f-constraints-1v1}
% \begin{aligned}
%     & \lambda_1 f_{\bm{x}}(\hat{\bm{x}}, X) = - \lambda_2 g_{\bm{y}}(\hat{\bm{y}}), \; \rho_{\bm{y}}	(\hat{\bm{x}}, \hat{\bm{y}}) = - \lambda_2 g_{\bm{y}}(\hat{\bm{y}}) \\
% 	& f(\hat{\bm{x}}, X) = 0, \; g(\hat{\bm{y}}) = 0, \; \lambda_1 < 0, \; \lambda_2 > 0.
% \end{aligned}
% \end{equation}
% Let $\xi_1 = - \frac{\lambda_2}{\lambda_1} > 0$ and $\xi_2 = \lambda_2 > 0$, and thus by replacing $\hat{\bm{x}}, \hat{\bm{y}}$ with $\bm{x}, \bm{y}$ respectively, \eqref{eq:f-constraints-1v1} becomes the constraints in \eqref{eq:optimization-pbm-set-1v1}, where $\rho_{\bm{y}}	(\hat{\bm{x}}, \hat{\bm{y}}) = \frac{\hat{\bm{y}} - \hat{\bm{x}}}{\|\hat{\bm{x}} -  \hat{\bm{y}}\|_2}$ is used. Then, we have $V^*_{N} \leq 0$ by combining \eqref{eq:simplified-f-max-1v1} and \eqref{eq:f-constraints-1v1}. 

% Let $\mathcal{X}_U \triangleq \mathcal{X} \cap \mathcal{C}_U$. We next consider $X$ in the universal subspace $\mathcal{X}_U$, i.e., $\theta_P = \sigma^u(\bm{x}_P, \bm{x}_E)$. According to condition \ref{itm:PEF-defi-2} in \defiref{defi:PEF}, $f(\hat{\bm{x}}, X) \equiv 0$ is reduced to $f^u(\hat{\bm{x}}, \bm{x}_P, \bm{x}_E) \equiv 0$, and $f^u$ is differentiable in $\bm{x}$, $\bm{x}_P$ and $\bm{x}_E$. Then, we have $f_{\bm{x}}(\hat{\bm{x}}, X) = f_{\bm{x}}^u (\hat{\bm{x}}, \bm{x}_P, \bm{x}_E)$ and
% \begin{equation}\label{eq:f-to-control-absorb-1v1}
% \begin{aligned}
% &\dod{}{t}f^u(\hat{\bm{x}}, \bm{x}_P, \bm{x}_E) =0 \Rightarrow - f_{\bm{x}}^{u \top} (\hat{\bm{x}}, \bm{x}_P, \bm{x}_E) \dod{\hat{\bm{x}}}{t}\\
% & = f_{P}^{u \top} (\hat{\bm{x}}, \bm{x}_P, \bm{x}_E) \dod{\bm{x}_{P}}{t} + f_{E}^{u \top} (\hat{\bm{x}}, \bm{x}_P, \bm{x}_E) \dod{\bm{x}_{E}}{t}\\
% & = v_P \bar{f}_{P}^{u} (\hat{\bm{x}}, \bm{x}_P, \bm{x}_E)  + v_E f_{E}^{u \top} (\hat{\bm{x}}, \bm{x}_P, \bm{x}_E) \bm{u}_E \\
% & = v_E \big( \alpha \bar{f}_{P}^{u} (\hat{\bm{x}}, \bm{x}_P, \bm{x}_E)  + f_{E}^{u \top} (\hat{\bm{x}}, \bm{x}_P, \bm{x}_E) \bm{u}_E \big).
% \end{aligned}
% \end{equation}
% By following the same argument \eqref{eq:max-min-partial-rho-1v1}-\eqref{eq:simplified-f-max-1v1}, $\od{}{t}{\varrho}(X; f) \ge 0$ for all $X \in \mathcal{X}_U$ is equivalent to
% \begin{equation}\label{eq:simplified-f-max-absorb-1v1}
%     \max_{X \in \mathcal{X}_U} \alpha \bar{f}_{P}^u (\hat{\bm{x}}, \bm{x}_P, \bm{x}_E) + \left\| f_E^u(\hat{\bm{x}}, \bm{x}_P, \bm{x}_E) \right\|_2 \leq 0.
% \end{equation}
% Similar to the argument \eqref{eq:f-constraints-1v1}, we have $V_{U}^* \leq 0$.

Case 2: $\bm{x}_I = \bm{x}_G$. This implies that $\mathbb{E}(X'_{cj}; f_c)$ is tangent to $\goal$ at the unique point $\bm{x}_I$. Then, the conclusion can be proved similarly by replacing $d_{\bm{x}} (\bm{x}_I, \bm{x}_G)$ with $\lambda_g g_{\bm{y}}(\bm{x}_G)$ in \eqref{itm:winning-KKT-1}, and replacing \eqref{itm:winning-KKT-2} with the constraint $\| \lambda_g g_{\bm{y}}(\bm{x}_G) \|_2 = 1$. \qed

\begin{rek}
    As the proof of \thomref{thom:nece-suff-no-closing-nv1} shows, the optimal value $V$ to the problem \eqref{eq:optimization-pbm-set-nv1} is the minimum speed of the enclosure region moving away from $\goal$ over $\mathcal{S}_{cj}$. Moreover, the nonlinear program \eqref{eq:optimization-pbm-set-nv1} can be largely simplified if the derivatives of the PEFs are easy to compute.  
\end{rek}
% By classifying the index set $s$ as in \eqref{eq:slack-condition}, 
% Then we have
% \begin{equation}\label{eq:constraints-x-y}
% \begin{aligned}
% 	&\bm{0}=\lambda_g g_{\bm{y}}(\bm{x}_G) + \sum\nolimits_{i \in c} \lambda_i f_{i, \bm{x}} (\bm{x}_I, X'_{ij})\\
% 	& f_i (\bm{x}_I, X'_{ij}) \ge 0, \ \lambda_i \leq 0, \ \lambda_i f_i (\bm{x}_I, X'_{ij}) = 0, i \in c \\
% 	& g(\bm{x}_G) = 0, \ \lambda_g > 0, \ \bm{x}_I = \bm{x}_G
% 	\end{aligned}
% \end{equation}
% where $\lambda_g$ and $\lambda_i$ are such that $\| \lambda_g g_{\bm{y}}(\bm{x}_G) \|_2 = 1$. Furthermore by the tangent property, we have
% \begin{equation}\label{eq:lim-partial-rho-1v1}
% \begin{aligned}
%    \lim_{\bm{x} \to \bm{x}_I, \bm{y} \to \bm{x}_G} \rho_{\bm{y}}(\bm{x}, \bm{y}) & = - \lambda_g g_{\bm{y}}(\bm{x}_G) \\
%   \lim_{\bm{x} \to \bm{x}_I, \bm{y} \to \bm{x}_G} \rho_{\bm{x}}(\bm{x}, \bm{y}) & = - \sum\nolimits_{i \in c} \lambda_i f_{i, \bm{x}} (\bm{x}_I, X'_{ij}).
% \end{aligned}
% \end{equation}
% % where $\lambda_4  > 0, \lambda_5 > 0$ are the normalization factors. 
% Then, the speed $ \od{}{t}{\varrho}(X'_{cj}; f_c)$ of moving away from $\goal$ at $\bm{x}_I = \bm{x}_G$ is computed as follows
% \begin{equation*}
% \begin{aligned}
% 	 \dod{}{t}{\varrho}(X'_{cj}; f_c) & =  \lim_{\bm{x} \to \bm{x}_I, \bm{y} \to \bm{x}_G} \dod{}{t}\rho\left( \bm{x}, \bm{y} \right) \\
% 	 & = \lim_{\bm{x} \to \bm{x}_I, \bm{y} \to \bm{x}_G} \big( \rho_{\bm{x}}^{\top}(\bm{x}, \bm{y}) \dot{\bm{x}}+ \rho_{\bm{y}}^{\top}(\bm{x}, \bm{y}) \dot{\bm{y}} \big) \\
% 	 & = - \sum\nolimits_{i \in c} \lambda_i f_{i, \bm{x}}^\top (\bm{x}_I, X'_{ij}) \dot{\bm{x}}_I
% \end{aligned}
% \end{equation*}
% where the third equality is due to \eqref{eq:lim-partial-rho-1v1} and the fact that $\bm{x}_G$ is always at the boundary of $\goal$, i.e., $g(\bm{x}_G) \equiv 0$ and thus $g_{\bm{y}}^{\top} (\bm{x}_G) \dot{\bm{x}}_G = 0$. Then, by following the same argument \eqref{eq:slack-condition}, \eqref{eq:varrho-to-f-nv1}, \eqref{eq:f-to-control-nv1} and \eqref{eq:max-min-partial-rho-nv1}, the conclusion can be proved similarly. \qed
% Let $\xi_1 = \lambda_3$ and by replacing $\hat{\bm{x}}, \hat{\bm{y}}$ with $\bm{x}, \bm{y}$ respectively, \eqref{eq:constraint-x-y-1v1} becomes the constraints in \eqref{eq:optimization-pbm-set-1v1}. Then, we have $V^*_{N} \leq 0$ by combining \eqref{eq:simplified-f-max-1v1} and \eqref{eq:constraint-x-y-1v1}. Similarly, we also have $V_{U}^* \leq 0$.

% The conclusion follows from the fact that the above proofs are necessary and sufficient.
% We conclude that if $V_{\mathcal{X}}^* = \max\{ V_{N}^{*}, V_{U}^{*}\} \leq 0$, then $\od{}{t}{\varrho}(X; f) \ge 0$ for all $X \in \mathcal{X}$. Moreover, if $V^*_{\mathcal{X}} \leq 0$ holds, the maximum operation in \eqref{eq:min-f-1v1} shows that if $X \in \mathcal{X}_N$, then $u_P(X) = -\textup{sgn}(f_{\theta}(\hat{\bm{x}}, X))$, where $\hat{\bm{x}} = \eta(X)$. If $X \in \mathcal{X}_U$, we have $\bm{e}_{\theta_P} = \sigma(\bm{x}_P, \bm{x}_E)$ and its derivative with respect to $t$ implies
% \begin{equation*}
% \begin{aligned}
%       \dot{\theta}_P R_{90} \bm{e}_{\theta_P}  & =  \dpd{\sigma(\bm{x}_P, \bm{x}_E)}{\bm{x}_P}  \dot{\bm{x}}_P + \dpd{\sigma(\bm{x}_P, \bm{x}_E)}{\bm{x}_E} \dot{\bm{x}}_E \Rightarrow \\
%       \frac{u_P}{\kappa}  R_{90} \bm{e}_{\theta_P} & = \dpd{\sigma(\bm{x}_P, \bm{x}_E)}{\bm{x}_P} \bm{e}_{\theta_P} + \frac{1}{\alpha} \dpd{\sigma(\bm{x}_P, \bm{x}_E)}{\bm{x}_E} \bm{u}_E
% \end{aligned}
% \end{equation*}
% from which we have the pursuit strategy in \eqref{eq:pursuit-strategy-1v1}.
\end{thom}


% For $\bm{x}, \bm{y} \in \mathbb{R}^2$, if $\bm{x} \neq \bm{y}$, define $e(\bm{x}, \bm{y}) = \frac{\bm{x} - \bm{y}}{\|\bm{x} - \bm{y}\|_2}$.



% \subsection{Pursuit strategies and parameters for two pursuers}
% We next consider strategies and parameters for two pursuers and one evader. For simplicity of description,  we assume two pursuers $P_1, P_2 \in \pteam$ (i.e., $s = \{1, 2\}$) with PEFs $f_1, f_2$, capture radii $r_1, r_2 > 0$ and minimum turning radii $\kappa_1, \kappa_2 > 0$, and their speed ratios $\alpha_1, \alpha_2 > 1$ over an evader $E \in \eteam$, respectively. The associated system state $Y = (\bm{x}_{P_1}, \theta_{P_1}, \bm{x}_{P_2}, \theta_{P_2}, \bm{x}_E) \in \mathcal{A}_2$ is also referred to as $Y = (X_1, X_2)$, where $X_i = (\bm{x}_{P_i}, \theta_{P_i}, \bm{x}_E)$ for $i \in c$, and $\mathcal{A}_2$ is the states with non-negative safe distance under $f_1$ and $f_2$.

% % $P_1, P_2 \in \pteam$ (i.e., $s = \{1, 2\}$) and $E_j \in \eteam$ are considered. Unless for clarity, the subscripts $s$ and $j$ are omitted in this section. 

% % Thus, we denote the notation $\alpha_{1j}$, $\alpha_{2j}$, $X_{cj}$, $\mathcal{A}_{sj}$ by $\alpha_{1}$, $\alpha_{2}$, $Y$, $\mathcal{A}_2$, respectively.




% \begin{thom}\label{thom:nece-suff-no-closing-2v1}{\rm (Necessary and sufficient conditions for no-approaching).}
% Given a set of states $\mathcal{Y} \subset \mathcal{A}_2$, $P_1$ and $P_2$ cooperatively achieve no-approaching winning against $E$ over $\mathcal{Y}$, if and only if $V_{\mathcal{Y},f_1,f_2}^* \leq 0$, where $V_{\mathcal{Y},f_1,f_2}^*$ is the optimal value of the problem
% \begin{equation}\label{eq:optimization-pbm-set-2v1}
%     \begin{aligned}
%       & \textup{maximize} & & \sum_{i = 1}^2 \frac{\xi_i \alpha_i }{\kappa_{i}} \big( \kappa_{i} \bar{f}_{i, \bm{y}} (\bm{x}, X_i) - \left |f_{i, \theta}(\bm{x}, X_i) \right| \big) \\
%       & & & + \Big\|\sum_{i=1}^2 \xi_i f_{i, \bm{z}}(\bm{x}, X_i) \Big\|_2 \\
%       & \textup{variables}&& \bm{x} \in \mathbb{R}^2, \; \bm{y} \in \mathbb{R}^2, \; Y = (X_1, X_2) \in \mathcal{Y}, \\
%       & & & \xi_1 \in \mathbb{R}_{\ge 0}, \; \xi_2 \in \mathbb{R}_{\ge 0}, \; \xi_3 \in \mathbb{R}_{> 0} \\
%       &\textup{subject to} & & f_1(\bm{x}, X_1) = 0, \; f_2(\bm{x}, X_2) = 0, \; g(\bm{y}) = 0, \; \\
%       & & & \xi_1 f_{1, \bm{x}}(\bm{x}, X_1) + \xi_2 f_{2, \bm{x}}(\bm{x}, X_2) = \xi_3 g_{\bm{y}}(\bm{y}), \\
%       & & & \bm{x} - \bm{y} = \xi_3 \left \|\bm{x} - \bm{y} \right \|_2 g_{\bm{y}}(\bm{y}).
%     \end{aligned}
% \end{equation}
% Moreover, if $V_{\mathcal{Y}, f_1, f_2}^* \leq 0$ holds, then the pursuit strategy
% \begin{equation}\label{eq:pursuit-strategy-2v1}
%     u_{P_i}(Y) = -\textup{sgn}(f_{i, \theta}(\eta(Y), X_i)), \ \forall\; Y \in \mathcal{Y}
% \end{equation}
% for $i = 1, 2$, can guarantee $V_{\mathcal{Y}, f_1, f_2}^* \leq 0$.

% Proof. \rm
% Consider $Y \in \mathcal{Y}$. Since $\mathcal{Y} \subset \mathcal{A}_2$, then $\varrho(Y; f_1, f_2)\ge0$, i.e., $\rho(\mathbb{E}(Y; f_1, f_2), \goal) \ge 0$. Since $\mathbb{E}(Y; f_1, f_2)$ is strictly convex and $\goal$ is convex, there exists a unique solution $(\hat{\bm{x}},\hat{\bm{y}}) \in \mathbb{E}(Y; f_1, f_2) \times \goal$ to $\mathcal{P}(Y)$ in \eqref{eq:convex-pbm-IG}. 

% Case 1: $\hat{\bm{x}} \neq \hat{\bm{y}}$. According to the KKT conditions, the solution $\left(\hat{\bm{x}}, \hat{\bm{y}} \right)$ satisfies
% \begin{equation}\label{eq:kkt-condition-2v1}
% \begin{aligned}
% 	&\bm{0}= \rho_{\bm{x}} \left(\hat{\bm{x}}, \hat{\bm{y}} \right) + \lambda_1 f_{1,\bm{x}} (\hat{\bm{x}}, X_1) + \lambda_2 f_{2,\bm{x}} (\hat{\bm{x}}, X_2),\\
% 	&\bm{0}= \rho_{\bm{y}} \left( \hat{\bm{x}}, \hat{\bm{y}} \right) + \lambda_3 g_{\bm{y}}(\hat{\bm{y}}),\\
% 	& f_1 ( \hat{\bm{x}}, X_1) \ge 0, \; f_2 ( \hat{\bm{x}}, X_2) \ge 0,\; g\left(\hat{\bm{y}}\right)\le 0, \; \lambda_1 \leq 0, \; \lambda_2 \leq 0, \\
% 	&  \lambda_3 \ge 0, \; \lambda_1 f_1\left(\hat{\bm{x}}, X_1 \right) = 0, \; \lambda_2 f_2 (\hat{\bm{x}}, X_2) = 0, \; \lambda_3 g (\hat{\bm{y}}) = 0,
% \end{aligned}
% \end{equation}
% where $\lambda_1, \lambda_2, \lambda_3 \in \mathbb{R}$ are the Lagrange multipliers. With regard to $\od{}{t}{\varrho}(Y; f_1, f_2)$, we have
% \begin{equation}\label{eq:varrho-to-f-2v1}
% \begin{aligned}
% 	 & \dod{}{t}{\varrho}(Y; f_1, f_2) =  \dod{}{t}\rho\left( \hat{\bm{x}},\hat{\bm{y}} \right) \\
% 	 & =  \rho_{\bm{x}}^{\top}(\hat{\bm{x}}, \hat{\bm{y}}) \dod{\hat{\bm{x}}}{t} + \rho_{\bm{y}}^{\top}(\hat{\bm{x}}, \hat{\bm{y}}) \dod{\hat{\bm{y}}}{t}\\
% 	 & = - \lambda_1 f_{1,\bm{x}}^{\top} (\hat{\bm{x}}, X_1) \dod{\hat{\bm{x}}}{t} - \lambda_2 f_{2,\bm{x}}^{\top} (\hat{\bm{x}}, X_2) \dod{\hat{\bm{x}}}{t} - \lambda_3 g_{\bm{y}}^{\top} (\hat{\bm{y}}) \dod{\hat{\bm{y}}}{t} \\
% 	& = - \lambda_1 f_{1,\bm{x}}^{\top} (\hat{\bm{x}}, X_1) \dod{\hat{\bm{x}}}{t} - \lambda_2 f_{2,\bm{x}}^{\top} (\hat{\bm{x}}, X_2) \dod{\hat{\bm{x}}}{t},
% \end{aligned}
% \end{equation}
% where the third equality follows from \eqref{eq:kkt-condition-2v1}, and the fourth equality follows because $\hat{\bm{y}}$ is always at the boundary of $\goal$, i.e., $g(\hat{\bm{y}}) \equiv 0$ and thus $g_{\bm{y}}^{\top} (\hat{\bm{y}}) \od{\hat{\bm{y}}}{t} = 0$. Also, $\lambda_3 > 0$ holds by $\hat{\bm{x}} \neq \hat{\bm{y}}$ in \eqref{eq:kkt-condition-2v1}.

% Suppose that $\lambda_1 < 0$ and $\lambda_2 < 0$. Thus, $\hat{\bm{x}}$ is always at the boundaries of $\mathbb{E}(X_1; f_1)$ and $\mathbb{E}(X_2; f_2)$, that is, $f_1(\hat{\bm{x}}, X_1) \equiv 0$ and $f_2(\hat{\bm{x}}, X_2) \equiv 0$. By the same argument \eqref{eq:f-to-control-1v1}, we have
% \begin{equation}\label{eq:f-to-control-2v1}
% \begin{aligned}
%     & - f_{i,\bm{x}}^\top (\hat{\bm{x}}, X_i) \dod{\hat{\bm{x}}}{t} = \frac{v_E}{\kappa_{i}} \big( \alpha_i \kappa_{i} \bar{f}_{i, \bm{y}} (\hat{\bm{x}}, X_i) \\
%     & \quad \qquad \quad + \alpha_i f_{i, \theta}(\hat{\bm{x}}, X_i) u_{P_i} + \kappa_{i} f_{i, \bm{z}}^\top (\hat{\bm{x}}, X_i) \bm{u}_E \big),
% \end{aligned}
% \end{equation}
% for $i \in \{1, 2\}$. By assumption, $P_1$ and $P_2$ cooperatively achieve no-approaching winning against $E$ over $\mathcal{Y}$, i.e., there exists a pair of pursuit strategies $(u_{P_1}, u_{P_2})$ such that $\od{}{t}{\varrho}(Y; f_1, f_2) \ge 0$ for all $Y \in \mathcal{Y}$, regardless of $\bm{u}_E$. Equivalently, we have
% \begin{equation} \label{eq:max-min-partial-rho-2v1}
%     \max_{u_{P_1}, u_{P_2} \in \mathbb{U}_P} \min_{\bm{u}_E \in \mathbb{U}_E, Y \in \mathcal{Y}} \dod{}{t}{\varrho}(Y; f_1, f_2) \ge 0,
% \end{equation}
% from which we have
% \begin{equation}\label{eq:min-f-2v1}
% \begin{aligned}
%      0 & \leq \max_{u_{P_1}, u_{P_2} \in \mathbb{U}_P} \min_{\bm{u}_E \in \mathbb{U}_E, Y \in \mathcal{Y}} \sum_{i = 1}^2 \big( - \lambda_i f_{i,\bm{x}}^{\top} (\hat{\bm{x}}, X_i) \dod{\hat{\bm{x}}}{t} \big)\\
%      & = \max_{u_{P_1}, u_{P_2} \in \mathbb{U}_P} \min_{\bm{u}_E \in \mathbb{U}_E, Y \in \mathcal{Y}} \sum_{i = 1}^2 \frac{\lambda_i v_E}{\kappa_{i}} \big( \alpha_i \kappa_{i} \bar{f}_{i, \bm{y}} (\hat{\bm{x}}, X_i) \\
%      & \qquad \qquad \qquad + \alpha_i f_{i, \theta}(\hat{\bm{x}}, X_i) u_{P_i} + \kappa_{i} f_{i, \bm{z}}^\top (\hat{\bm{x}}, X_i) \bm{u}_E \big) \\
%      & = \min_{Y \in \mathcal{Y}} \Big( \sum_{i = 1}^2 \frac{\lambda_i \alpha_i v_E}{\kappa_{i}} \big(  \kappa_{i} \bar{f}_{i, \bm{y}} (\hat{\bm{x}}, X_i) - \left |f_{i, \theta}(\hat{\bm{x}}, X_i) \right| \big) \\
%      & \qquad \qquad \qquad - \Big\|\sum_{i=1}^2 \lambda_i v_E f_{i, \bm{z}}(\hat{\bm{x}}, X_i) \Big\|_2 \Big),
% \end{aligned}
% \end{equation}
% where the first inequality is due to \eqref{eq:varrho-to-f-2v1}, and the first equality follows from \eqref{eq:f-to-control-2v1}. In view of $\lambda_1 < 0$, $\lambda_2 < 0$ and $\lambda_3 > 0$, \eqref{eq:kkt-condition-2v1} is equivalent to
% \begin{equation}\label{eq:f-constraints-2v1}
% \begin{aligned}
% 	& \lambda_1 f_{1,\bm{x}} (\hat{\bm{x}}, X_1) + \lambda_2 f_{2,\bm{x}} (\hat{\bm{x}}, X_2) = - \lambda_3 g_{\bm{y}}(\hat{\bm{y}}) \\
% 	& \rho_{\bm{y}} \left( \hat{\bm{x}}, \hat{\bm{y}} \right) =  - \lambda_3 g_{\bm{y}}(\hat{\bm{y}}), \; f_1 ( \hat{\bm{x}}, X_1) = 0, \\
% 	& f_2 ( \hat{\bm{x}}, X_2) = 0, \; g\left(\hat{\bm{y}}\right) = 0, \; \lambda_1 < 0, \; \lambda_2 < 0, \; \lambda_3 > 0,
% \end{aligned}
% \end{equation}
% Let $\xi_1 = - \lambda_1 > 0$, $\xi_2 = - \lambda_2 > 0$ and $\xi_3 = \lambda_3 > 0$, and thus by replacing $\hat{\bm{x}}, \hat{\bm{y}}$ with $\bm{x}, \bm{y}$ respectively, \eqref{eq:f-constraints-2v1} becomes the constraints in \eqref{eq:optimization-pbm-set-2v1}, where $\rho_{\bm{y}}	(\hat{\bm{x}}, \hat{\bm{y}}) = \frac{\hat{\bm{y}} - \hat{\bm{x}}}{\|\hat{\bm{x}} -  \hat{\bm{y}}\|_2}$ is used. Therefore, we have $V^*_{\mathcal{Y}, f_1, f_2} \leq 0$ by combining \eqref{eq:min-f-2v1} and \eqref{eq:f-constraints-2v1}.

% If $\lambda_1 = 0$ or $\lambda_2 = 0$ ($\lambda_1 = \lambda_2 = 0$ does not hold as $\hat{\bm{x}} \neq \hat{\bm{y}}$ in \eqref{eq:kkt-condition-2v1}), then \eqref{eq:varrho-to-f-2v1} is degenerated into the one-pursuer case as in \eqref{eq:varrho-to-f-1v1}. The results directly follow from the same argument in the proof of \thomref{thom:nece-suff-no-closing-1v1}.

% Case 2: $\hat{\bm{x}} = \hat{\bm{y}}$. Suppose that $\lambda_1 < 0$ and $\lambda_2 < 0$.Then, $\hat{\bm{x}}$ is always at the boundaries of $\mathbb{E}(X_1; f_1)$ and $\mathbb{E}(X_2; f_2)$. This implies that $\mathbb{E}(X_1; f_1)$ and $\mathbb{E}(X_2; f_2)$ are both tangent to $\goal$ at the unique point $\hat{\bm{x}}$, and then it follows that
% \begin{equation}
% \begin{aligned}
%     & f_1(\hat{\bm{x}}, X_1) = 0, f_2(\hat{\bm{x}}, X_2) = 0, g(\hat{\bm{y}}) = 0,  \hat{\bm{x}} = \hat{\bm{y}}, \\
%     & f_{1,\bm{x}}(\hat{\bm{x}}, X_1) = \lambda_4 g_{\bm{y}}(\hat{\bm{y}}), f_{2,\bm{x}}(\hat{\bm{x}}, X_2) = \lambda_5 g_{\bm{y}}(\hat{\bm{y}}),
% \end{aligned}
% \end{equation}
% where $\lambda_4 > 0$ and $\lambda_5 > 0$. Then, the results follow from the same argument \eqref{eq:lim-partial-rho-1v1} and \eqref{eq:deri-x=y-1v1} for one pursuer. For $\lambda_1 = 0$ or $\lambda_2 = 0$, we prove it similarly as it is degenerated into one-pursuer case.
% \qed 
% \end{thom}



